Completeness for Probabilistic Boolean Tapes

Probabilistic Boolean circuits have recently been proposed as a string-diagrammatic foundation for finite probabilistic programming. In this paper, we present a complete set of axioms for their semantics in terms of Markov kernels. Our approach is based on two intermediate results: completeness for \emph{partial} Boolean circuits and completeness for probabilistic Boolean tapes, a diagrammatic language for rig categories.

==> appendices/appcompletenessprobtapes-NEW.tex <==
\section{Appendix of Section \ref{sec:completenessprobbooltapes-NEW}}\label{app:{sec:completenessprobbooltapes-NEW}}



\begin{proof}[Proof of Proposition \ref{prop:soundnesstapes}]
  %\marginpar{CIPRIANO CHECK: - OK}
Since the axioms in $\ThPB$ are sounds with respect to $\osem{-}$ and since $\osem{-}=\dsem{\encoding{-}}$, these axioms are also sound for $\dsem{-}$.
For \eqref{ax:AXPBP1} and \eqref{ax:AXPBP2}, it enough to check that the left and the right hand sides are mapped into the same $\KlD$-arrows by $\dsem{-}$.
For \eqref{ax:canc}, it is enough to observe that cancellativity holds in $\KlD$.
\end{proof}


Consider the congruence $\tapeeqPB$ on $\CatT{\Diag{\SigPB}}$ generated by the rules in \eqref{eq:congr2}
\begin{equation}\label{eq:congr2}
        \scalebox{0.85}{$
        \centering
        \begin{array}{c}
        \begin{array}{c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c}
            \inferrule*[right=($\ThPB$)]{c =_{\ThPB} d}{\tape{c} \tapeeqPB \tape{d}}
            &
            \inferrule*[right=($\textsc{R}$)]{-}{\t \tapeeqPB \t}
            &
            \inferrule*[right=($\textsc{S}$)]{\t_1 \tapeeqPB \t_2}{\t_2 \tapeeqPB \t_1}
            &    
            \inferrule*[right=($\textsc{T}$)]{\t_1 \tapeeqPB \t_2 \quad \t_2 \tapeeqPB \t_3}{\t_1 \tapeeqPB \t_3}
            % &
            % \inferrule*[right=($E$)]{ (t,t') \in E \and U \in \sort^\star}{ t_U \tapeeqPB t'_U}
        \end{array}
        \\[10pt]
        \begin{array}{c@{\qquad}c@{\qquad}c}
            \inferrule*[right=($;$)]{\t_1 \tapeeqPB \t_2 \quad \s_1 \tapeeqPB \s_2}{\t_1;\s_1 \tapeeqPB \t_2;\s_2}
            &
            \inferrule*[right=($\piu$)]{\t_1 \tapeeqPB \t_2 \quad \s_1 \tapeeqPB \s_2}{\t_1\piu\s_1 \tapeeqPB \t_2 \piu \s_2}
            &
            \inferrule*[right=($\per $)]{\t_1 \tapeeqPB \t_2 \quad \s_1 \tapeeqPB \s_2}{\t_1\per \s_1 \tapeeqPB \t_2 \per \s_2}       
        \end{array}
        \end{array}
        $}
\end{equation}

\begin{proposition}\label{prop:quotienttheory}
For all $\s , \t \in \CatT{\Diag{\SigPB}}$, $\s \tapeeqPB \t$ iff $\CatT{Q_{\ThPB}}(\s) = \CatT{Q_{\ThPB}}(\t)$.
\end{proposition}
\begin{proof}
  Let $\CatT{\Diag{\SigPB}}_{\tapeeqPB}$ be the quotient of $\CatT{\Diag{\SigPB}}$ by $\tapeeqPB$: objects are those of  $\CatT{\Diag{\SigPB}}$, arrows are $\tapeeqPB$-equivalence classes of arrows of $\CatT{\Diag{\SigPB}}$, hereafter denoted by $[\t]_{\tapeeqPB}$. We prove that $\CatT{\Diag{\SigPB}}_{\tapeeqPB}$ is isomorphic to $\CatT{\Diag{\ThPB}}$.

We first define the functor $F \colon \CatT{\Diag{\SigPB}}_{\tapeeqPB} \to \CatT{\Diag{\ThPB}}$ inductively as
\[\begin{array}{ccccc}
F(\diagp{U})\defeq \; \diagp{U} &  F(\,\bangp{U})\defeq \bangp{U} & F(\tapeFunct{c})\defeq \tapeFunct{[c]_{\ThPB}} &  F(\cobang{U})\defeq \cobang{U} &
F(\codiag{U})\defeq\codiag{U}  \\
 F(\id{U})\defeq \id{U} & F(\id{\zero})\defeq\id{\zero} & F(\sigma_{U,V}^{\piu})\defeq \sigma_{U,V}^{\piu}& F(\t_1 ; \t_2)\defeq F(\t_1);F(\t_2) & F(\t_1 \piu \t_2) \defeq F(\t_1)\piu F(\t_2)
\end{array}\]
Since arrows in $\CatT{\Diag{\SigPB}}_{\tapeeqPB}$ are $\tapeeqPB$-equivalence classes, we need to prove that the functor is well-defined, namely that if $\s \tapeeqPB  \t$ then $F(\s)=F(\t)$. This is done by induction on the rules in \eqref{eq:congr2}. For the case of the rule ($\ThPB$), observe that $\s=\tape{c}$, $\t=\tape{d}$ and $c=_{\ThPB}d$. By the definition of $F$, $F(\s)=F(\t)$. All the other cases are trivial, with the only exception of the rule $(\otimes)$ where one observes that, since  $=_{\ThPB}$ is a congruence w.r.t. $\otimes$, then $F$ is a morphism of rig categories.

The functor  $G \colon  \CatT{\Diag{\ThPB}} \to \CatT{\Diag{\SigPB}}_{\tapeeqPB} $ is defined on $\tapeFunct{[c]_{\ThPB}}$ as $G(\tapeFunct{[c]_{\ThPB}})\defeq [\tapeFunct{c}]_{\tapeeqPB}$ and then inductively in the same style of the functor $F$ above. Observe that $F(G(\tapeFunct{[c]_{\ThPB}}))=\tapeFunct{[c]_{\ThPB}}$ and $G(F([\tapeFunct{c}]_{\tapeeqPB})) = [\tapeFunct{c}]_{\tapeeqPB}$. A simple inductive argument confirms that $F$ and $G$ are inverses of each other.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:twoequivalence}]
 
  We first prove by induction on the rules in \eqref{eq:congr3} that if $\s \dot{\sim} \t$ then $\CatT{Q_{\ThPB}}(\s) \eqsyn \CatT{Q_{\ThPB}}(\t)$.
Consider the case of the rule $(\ThPB)$: in this case $\s=\tapeFunct{c}$, $\t=\tapeFunct{d}$ and $c\eqPB d$. Thus $\CatT{Q_{\ThPB}}(\s)= \CatT{Q_{\ThPB}}(\t)$.
All the other cases trivially follow from the fact that $\CatT{Q_{\ThPB}}$ is a morphism of rig categories: see \cite{bonchi2025tapediagramsmonoidalmonads}.

Again, by induction on the rules, we prove that if $\CatT{Q_{\ThPB}}(\s) \eqsyn \CatT{Q_{\ThPB}}(\t)$ then $\s \dot{\sim} \t$.
Here the only non-trivial cases are $(R)$, $\eqref{ax:AXPBP1}$ and $\eqref{ax:AXPBP2}$. For $(R)$, if $\CatT{Q_{\ThPB}}(\s) = \CatT{Q_{\ThPB}}(\t)$, then by Proposition \ref{prop:quotienttheory}, $\s \tapeeqPB \t$. Hence, $\s \dot{\sim} \t$. For $\eqref{ax:AXPBP1}$, if $\CatT{Q_{\ThPB}}(\s) \overset{\eqref{ax:AXPBP1}}{=} \CatT{Q_{\ThPB}}(\t)$, then $\s$ is $\tapeeqPB$-equivalent to the left hand side of \eqref{ax:AXPBP1} and $\t$ is $\tapeeqPB$-equivalent to the right hand side of \eqref{ax:AXPBP1}. Hence, they are $\dot{\sim}$-equivalent, and applying transitivity of $\dot{\sim}$, we conclude that $\s \dot{\sim} \t$. The case of $\eqref{ax:AXPBP2}$ is analogous.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:bottomstar2}]
 \begin{align}
  \Flipn{\bot}[t]&=\Flip{\bot}[t] ;\ncopierbis[t]  \tag{Def.\ of $\Flipn{\bot}$}\\
  &\sim \Tcounitempty{};\Tunit{}; \ncopierbis[t]  \tag{Axiom \ref{ax:AXPBP2}}\\
  &=  \Tcounitempty{};\Tunitm{n} \tag{\eqref{ax:tapes:cobangnat}}\\
  &= \star_{A^0,A^n}. \tag{Def. of $\star$}
 \end{align}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:PBP2}]
Consider the following derivation: 
\begin{align}
  \frac{1}{2^n} \cdot \t &= \frac{1}{2^n}\cdot (\id{A^n};\t) \notag\\
  &= (\frac{1}{2^n}\cdot \id{A^n});\t \tag{$\Cat{PCA}$-enrichment} \\ 
  &\sim (\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b});\t \tag{Lemma \ref{lemma:axiomsninput}}\\
  &= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b};\t \tag{\eqref{eq:enr}}\\
  &\sim \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b};\s \tag{Hp.}\\
  &=(\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b});\s \tag{\eqref{eq:enr}}\\
  &\sim (\frac{1}{2^n}\cdot \id{A^n});\s \tag{Lemma \ref{lemma:axiomsninput}}\\
  &= \frac{1}{2^n} \cdot \s. \tag{$\Cat{PCA}$-enrichment} 
\end{align}
Hence, applying axiom \eqref{ax:canc}, we conclude that $\t \eqsyn \s$.
\end{proof}

\begin{proof}[proof of Lemma~\ref{lemma:axiomsninput}]
By induction  on $n$. The base case is trivial. For the inductive step, we have
 \begin{align}
  \frac{1}{2^{n+1}}\cdot \id{A^{n+1}}&= \frac{1}{2^n}\frac{1}{2}\cdot( \id{A}\otimes \id{A^n}) \notag\\
  &= \frac{1}{2^n}\cdot\left(\frac{1}{2}\cdot \id{A}\otimes \id{A^n} \right) \tag{\eqref{eq:monoidalenrichment}}\\
  &= (\frac{1}{2}\cdot \id{A})\otimes (\frac{1}{2^n}\cdot \id{A^n}) \tag{\eqref{eq:monoidalenrichment}}\\
  &\sim (\frac{1}{2}\cdot \id{A})\otimes \left(\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b}\right) \tag{Inductive hypothesis}\\
  &\sim (\coflip{1}[t];\Flip{1}[t] +_{\frac{1}{2}} \coflip{0}[t];\Flip{0}[t]) \otimes \left(\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b}\right) \tag{Axiom \ref{ax:AXPBP1}}\\
  &= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\left((\coflip{1}[t];\Flip{1}[t] +_{\frac{1}{2}} \coflip{0}[t];\Flip{0}[t]) \otimes (\overleftarrow{b};\overrightarrow{b})\right) \tag{\eqref{eq:monoidalenrichment}}\\
  &=\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\left(((\coflip{1}[t];\Flip{1}[t]) \otimes (\overleftarrow{b};\overrightarrow{b})) +_{\frac{1}{2}} ((\coflip{0}[t];\Flip{0}[t]) \otimes (\overleftarrow{b};\overrightarrow{b}))\right) \tag{SMC}\\
  &= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\left((\coflip{1}[t]\otimes \overleftarrow{b});(\Flip{1}[t]\otimes \overrightarrow{b}) +_{\frac{1}{2}} (\coflip{0}[t]\otimes \overleftarrow{b});(\Flip{0}[t]\otimes \overrightarrow{b})\right) \tag{\eqref{eq:monoidalenrichment}}
 \end{align}
 Now, since the set $\{\Flip{1}[t]\otimes \overrightarrow{b}, \Flip{0}[t]\otimes \overrightarrow{b}\}$ as $\overrightarrow{b}\in \Cat{B}[1,A^n]$ is exactly $\Cat{B}[1,A^{n+1}]$, then, rearranging the above sum we obtain $\frac{1}{2^{n+1}}\cdot \id{A^{n+1}}= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^{n+1}]}^{} \frac{1}{2^{n+1}}\cdot\overleftarrow{b};\overrightarrow{b}$, as desired.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lemma:diagramma-commutativo}]
    TBA
    \end{proof}


\begin{proof}[Proof of Lemma \ref{lemma:Ffaith}]
  Since $\ParJ_2'=\stmat{\ParJ_2^\sharp}\circ \epsilon$ and we have the isomorphism $\stmat{\Cat{Par}_2^+}[A^0,A^m]\cong \Cat{Par}_2^+[A^0,A^m]$, we prove that $\ParJ_2^\sharp\colon\Cat{Par}_2^+
   \to \KlD$ is faithful when restricted to $\Sets_2^+[1,2^m]$. Now recall from Theorem~\ref{thm:freeenriched} that $\ParJ_2^\sharp$ is the identity-on-objects functor sending a subdistribution $d\in \Cat{Par}_2^+[1,2^m]$ into the subdistribution $\ParJ_2^\sharp(d)= \sum_{f\in \Cat{Par}_2[1,2^m]} d(f)\cdot{\ParJ_2(f)}$. Hence, if $d\in \Sets_2^+[1,2^m]$, then $\ParJ_2^\sharp(d)= \sum_{f\in \Sets_2[1,2^m]} d(f)\cdot{\ParJ_2(f)}=\sum_{f\in \Sets_2[1,2^m]} d(f)\cdot{\delta_{f(\bullet)}}$, where $f(\bullet)\in 2^m$. Hence, $\ParJ_2^\sharp$ restricted to $\Sets_2^+[1,2^m]$ provides the obvious bijection $$\Dis(\Sets_2[1,2^m])\cong \Dis(2^m) \cong   \KlD_2[1,2^m]\text{.}$$ 
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:PBP0}]
Since $\CatT{\Diag{\ThPB}}\cong \stmat{\Diag{\ThPB}^+}$,  $\t$ corresponds to  a subdistribution on $\Diag{\ThPB}[A^0,A^m]$. By Lemma~\ref{lemma:caratterizzazionecircuiti0n}, each partial Boolean circuit in $\Diag{\ThPB}[A^0,A^m]$ is either a Boolean circuit in $\Diag{\SigB}[1,A^m]$ or it is of the form $\Flipm{\bot}$. Hence, we can rearrange the subdistribution corresponding to $\t$ into a tape of the desired form.
\end{proof}



\begin{proof}[Proof of Lemma \ref{lemma:PBP1}]
  By Lemma~\ref{lemma:PBP0}, we can write 
  \begin{equation}\label{eq:BLABLA}
  \t=(\sum_{i=1}^{n}p_i\cdot b_i)+_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t]) \text{ and }\t'=(\sum_{j=1}^{n'}p'_j\cdot b'_j)+_{p'}(\star_{A^0,A^m} +_{q'} \Flipm{\bot}[t])\end{equation} 
  for some $p_i,p'_j\in (0,1)$, for $i=1,\dots,n$ and $j=1,\dots,n'$, $p,p',q,q'\in [0,1]$  such that $\sum_{i=1}^{n}p_i= 1$ and $\sum_{j=1}^{n'}p'_j= 1$, where $b_i\colon A^0 \to A^m\in \Cat{B}[1,A^m]$ and $b'_j\colon A^0 \to A^m\in \Cat{B}[1,A^m]$. Then,
  \begin{align}
    \ParJ_2'\circ \iso(\t)&= \ParJ_2'\circ \iso((\sum_{i=1}^{n}p_i\cdot b_i) +_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t])) \tag{\eqref{eq:BLABLA}}\\
    &= \ParJ_2'\circ \iso((\sum_{i=1}^{n}p_i\cdot b_i)) +_p(\ParJ_2'\circ \iso(\star_{A^0,A^m}) +_q \ParJ_2'\circ \iso(\Flipm{\bot}[t])) \tag{$\ParJ_2'$ pca-enriched}\\
    &= \ParJ_2'\circ \iso((\sum_{i=1}^{n}p_i\cdot b_i)) +_p (\star_{1,2^m} +_q \star_{1,2^m}) \tag{$\ParJ_2^\sharp(\star_{2^0,2^m})=\star_{1,2^m}=\ParJ_2^\sharp(\delta_\bot)$}\\
    &= p\cdot \ParJ_2'\circ \iso(\sum_{i=1}^{n}p_i\cdot b_i) \tag{Idemp.\ in (\ref{eq:pca})}\\
    &=\ParJ_2'\circ \iso(p\cdot \sum_{i=1}^{n}p_i\cdot b_i)\tag{$\ParJ_2'$ pca-enriched}
  \end{align}
  and similarly $\ParJ_2'\circ \iso(\t')=\ParJ_2'\circ \iso(p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j)$. Hence, $\ParJ_2'\circ \iso(p\cdot \sum_{i=1}^{n}p_i\cdot b_i)=\ParJ_2'\circ \iso(p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j)$, and Lemma~\ref{lemma:Ffaith} implies that  
  \begin{equation}\label{BLA2}p\cdot \sum_{i=1}^{n}p_i\cdot b_i=p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j\text{.}\end{equation} Thus,
  \begin{align}
    \t&=(\sum_{i=1}^{n}p_i\cdot b_i) +_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t]) \tag{\eqref{eq:BLABLA}}\\
    &\sim  \sum_{i=1}^{n}p_i\cdot b_i +_p(\star_{A^0,A^m} +_q \star_{A^0,A^m}) \tag{Lemma \ref{lemma:bottomstar2}}\\
    &= \sum_{i=1}^{n}p_i\cdot b_i +_p \star_{A^0,A^m} \tag{Idemp.\ in (\ref{eq:pca})}\\
    &= p\cdot \sum_{i=1}^{n}p_i\cdot b_i\tag{Def. $p\cdot-$}\\
    &= p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j \tag{\eqref{BLA2}}\\
    &= \sum_{j=1}^{n'}p'_j\cdot b'_j +_{p'} \star_{A^0,A^m} \tag{Def. $p\cdot-$}\\
    &\sim \sum_{j=1}^{n'}p'_j\cdot b'_j +_{p'}(\star_{A^0,A^m} +_{q'} \star_{A^0,A^m}) \tag{Idemp.\ in (\ref{eq:pca})}\\
    &= \sum_{j=1}^{n'}p'_j\cdot b'_j +_{p'}(\star_{A^0,A^m} +_{q'} \Flipm{\bot}[t]) \tag{Lemma \ref{lemma:bottomstar2}}\\
    &= \t'. \tag{\eqref{eq:BLABLA}}
  \end{align}
\end{proof}



\begin{proof}[Additional details for the proof of Theorem~\ref{thm:completenessPBPtapes}]
    In the main text we have already proved that $I$ is faithful for arrows of type $A^n \to A^m$.
     This fact and convex products easily entail that $I$ is faithful for arrows $\s,\t \colon A^k \to \bigoplus_{i=1}^nA^{m_i}$. 
Indeed, by Theorem~\ref{thm:TCconvexbiproductcategory}, 
\begin{equation}\label{eq:boh}\s=\langle \s_1, \dots, \s_n \rangle_{\vec{q}} \quad \t=\langle \t_1, \dots, \t_n \rangle_{\vec{p}}\end{equation} 
for some $\vec{q}=q_1,\dots, q_n$, $\vec{p}=p_1,\dots, p_n$, $\s_i \colon A^k \to A^{m_i}$ and $\t_i \colon A^k \to A^{m_i}$. Thus
\begin{align*}
I([\s]_\eqsyn) = I([\t]_\eqsyn) & \Rightarrow \ParJ'_2(\iso(\s))=\ParJ'_2(\iso(\t)) \tag{$\ParJ'_2\circ \iso=I \circ\eqsynq{Q}$}\\
& \Rightarrow \text{for all }j \text{, } \ParJ'_2(\iso(\s));\ParJ'_2(\iso(\pi_j))=\ParJ'_2(\iso(\t));\ParJ'_2(\iso(\pi_j)) \\
& \Rightarrow \text{for all }j\text{, } \ParJ'_2(\iso(\s;\pi_j))=\ParJ'_2(\iso(\t;\pi_j)) \tag{Functoriality} \\
& \Rightarrow  \text{for all }j\text{, }  \s;\pi_j\sim\t;\pi_j \tag{Previous implication}\\
& \Rightarrow  \text{for all }j\text{, }  q_j \cdot \s_j\sim p_j \cdot \t_j \tag{\ref{eq:boh}}\\
& \Rightarrow  \text{for all }j\text{, }  [q_j \cdot \s_j]_\sim = [p_j \cdot \t_j]_\sim 
\end{align*}
%To conclude that $[\s]_\sim=[\t]_\sim$, observe that 
Now \cite[Proposition 6]{probbooltapesfossacs} states that $\CatT{\Diag{\ThPB}}_\sim$ is a convex biproduct category and that the quotient functor $Q_\eqsyn\colon \CatT{\Diag{\ThPB}} \to \CatT{\Diag{\ThPB}}_\sim$ is a morphism of convex biproduct categories.  Hence, \cite[Corollary 4]{arxivprobbooltapes} implies that $(\bigoplus_{j=1}^nA^{m_j}, [\pi_j]_\sim)$ is the $n$-ary convex product of $A^{m_1}, \dots, A^{m_n}$ in $\CatT{\Diag{\ThPB}}_\sim$ and $ [\s]_\sim$ is the unique arrow such that for all $j=1,\dots,n$,
\begin{align}
 [\s]_\sim;[\pi_j]_\sim &= [\s;\pi_j]_\sim \tag{Functoriality of $Q_\eqsyn$}\\
  &=[q_j \cdot \s_j]_\sim \tag{\ref{eq:boh}}\\
 &=q_j\cdot [\s_j]_\sim; \tag{pca-enrichment of $\CatT{\Diag{\ThPB}}_\sim$}
\end{align}
while $[\t]_\sim$ is the unique arrow such that for all $j=1,\dots,n$,
\begin{align}
  [\t]_\sim;[\pi_j]_\sim&= [\t;\pi_j]_\sim \tag{Functoriality of $Q_\eqsyn$}\\
  &= [p_j \cdot \t_j]_\sim \tag{\ref{eq:boh}}\\
  &=p_j\cdot [\t_j]_\sim. \tag{pca-enrichment of $\CatT{\Diag{\ThPB}}_\sim$}
\end{align}
Hence, since for all $j=1,\dots,n$, $[q_j \cdot \s_j]_\sim = [p_j \cdot \t_j]_\sim$, we have $[\s]_\sim = [\t]_\sim$.

%$[\s]_\sim=\langle [\s_1]_\sim, \dots, [\s_n]_\sim \rangle_{\vec{q}}$ and $[\t]_\sim=\langle [\t_1]_\sim, \dots, [\t_n]_\sim \rangle_{\vec{p}}$. Since for all $i$, $[\t];[\pi_i]_\sim$ and  $[\s];[\pi_i]_\sim$ are both equal to  $p_i\cdot[\t_i]_\sim=[p_i \cdot \t_i]_\sim=[q_i \cdot \s_i]_\sim$, the universal  property of  n-ary convex products in $\CatT{\Diag{\ThPB}}_\sim$ implies that $[\s]_\sim=[\t]_\sim $.

For arrows of arbitrary type $\bigoplus_{j=1}^o A^{k_j} \to \bigoplus_{i=1}^nA^{m_i}$, one can easily rely on the universal property of coproducts and the case that we just proved.
\end{proof}

==> appendices/appcompletenessprobtapes.tex <==
\section{Appendix to Section~\ref{sec:completenessprobbooltapes}}\label{app:{sec:completenessprobbooltapes}}

\begin{proof}[Proof of Proposition \ref{prop:soundnesstapes}]
  %\marginpar{CIPRIANO CHECK: - OK}
Since the axioms in $\ThPB$ are sounds with respect to $\osem{-}$ and since $\osem{-}=\dsem{\encoding{-}}$, these axioms are also sound for $\dsem{-}$.
For \eqref{ax:AXPBP1} and \eqref{ax:AXPBP2}, it enough to check that the left and the right hand sides are mapped into the same $\KlD$-arrows by $\dsem{-}$.
For \eqref{ax:canc}, it is enough to observe that cancellativity holds in $\KlD$.
\end{proof}


Consider the congruence $\tapeeqPB$ on $\CatT{\Diag{\SigPB}}$ generated by the rules in \eqref{eq:congr2}
\begin{equation}\label{eq:congr2}
        \scalebox{0.85}{$
        \centering
        \begin{array}{c}
        \begin{array}{c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c}
            \inferrule*[right=($\ThPB$)]{c =_{\ThPB} d}{\tape{c} \tapeeqPB \tape{d}}
            &
            \inferrule*[right=($\textsc{R}$)]{-}{\t \tapeeqPB \t}
            &
            \inferrule*[right=($\textsc{S}$)]{\t_1 \tapeeqPB \t_2}{\t_2 \tapeeqPB \t_1}
            &    
            \inferrule*[right=($\textsc{T}$)]{\t_1 \tapeeqPB \t_2 \quad \t_2 \tapeeqPB \t_3}{\t_1 \tapeeqPB \t_3}
            % &
            % \inferrule*[right=($E$)]{ (t,t') \in E \and U \in \sort^\star}{ t_U \tapeeqPB t'_U}
        \end{array}
        \\[10pt]
        \begin{array}{c@{\qquad}c@{\qquad}c}
            \inferrule*[right=($;$)]{\t_1 \tapeeqPB \t_2 \quad \s_1 \tapeeqPB \s_2}{\t_1;\s_1 \tapeeqPB \t_2;\s_2}
            &
            \inferrule*[right=($\piu$)]{\t_1 \tapeeqPB \t_2 \quad \s_1 \tapeeqPB \s_2}{\t_1\piu\s_1 \tapeeqPB \t_2 \piu \s_2}
            &
            \inferrule*[right=($\per $)]{\t_1 \tapeeqPB \t_2 \quad \s_1 \tapeeqPB \s_2}{\t_1\per \s_1 \tapeeqPB \t_2 \per \s_2}       
        \end{array}
        \end{array}
        $}
\end{equation}

\begin{proposition}\label{prop:quotienttheory}
For all $\s , \t \in \CatT{\Diag{\SigPB}}$, $\s \tapeeqPB \t$ iff $\CatT{Q_{\ThPB}}(\s) = \CatT{Q_{\ThPB}}(\t)$.
\end{proposition}
\begin{proof}
  Let $\CatT{\Diag{\SigPB}}_{\tapeeqPB}$ be the quotient of $\CatT{\Diag{\SigPB}}$ by $\tapeeqPB$: objects are those of  $\CatT{\Diag{\SigPB}}$, arrows are $\tapeeqPB$-equivalence classes of arrows of $\CatT{\Diag{\SigPB}}$, hereafter denoted by $[\t]_{\tapeeqPB}$. We prove that $\CatT{\Diag{\SigPB}}_{\tapeeqPB}$ is isomorphic to $\CatT{\Diag{\ThPB}}$.

We first define the functor $F \colon \CatT{\Diag{\SigPB}}_{\tapeeqPB} \to \CatT{\Diag{\ThPB}}$ inductively as
\[\begin{array}{ccccc}
F(\diagp{U})\defeq \; \diagp{U} &  F(\,\bangp{U})\defeq \bangp{U} & F(\tapeFunct{c})\defeq \tapeFunct{[c]_{\ThPB}} &  F(\cobang{U})\defeq \cobang{U} &
F(\codiag{U})\defeq\codiag{U}  \\
 F(\id{U})\defeq \id{U} & F(\id{\zero})\defeq\id{\zero} & F(\sigma_{U,V}^{\piu})\defeq \sigma_{U,V}^{\piu}& F(\t_1 ; \t_2)\defeq F(\t_1);F(\t_2) & F(\t_1 \piu \t_2) \defeq F(\t_1)\piu F(\t_2)
\end{array}\]
Since arrows in $\CatT{\Diag{\SigPB}}_{\tapeeqPB}$ are $\tapeeqPB$-equivalence classes, we need to prove that the functor is well-defined, namely that if $\s \tapeeqPB  \t$ then $F(\s)=F(\t)$. This is done by induction on the rules in \eqref{eq:congr2}. For the case of the rule ($\ThPB$), observe that $\s=\tape{c}$, $\t=\tape{d}$ and $c=_{\ThPB}d$. By the definition of $F$, $F(\s)=F(\t)$. All the other cases are trivial, with the only exception of the rule $(\otimes)$ where one observes that, since  $=_{\ThPB}$ is a congruence w.r.t. $\otimes$, then $F$ is a morphism of rig categories.

The functor  $G \colon  \CatT{\Diag{\ThPB}} \to \CatT{\Diag{\SigPB}}_{\tapeeqPB} $ is defined on $\tapeFunct{[c]_{\ThPB}}$ as $G(\tapeFunct{[c]_{\ThPB}})\defeq [\tapeFunct{c}]_{\tapeeqPB}$ and then inductively in the same style of the functor $F$ above. Observe that $F(G(\tapeFunct{[c]_{\ThPB}}))=\tapeFunct{[c]_{\ThPB}}$ and $G(F([\tapeFunct{c}]_{\tapeeqPB})) = [\tapeFunct{c}]_{\tapeeqPB}$. A simple inductive argument confirms that $F$ and $G$ are inverses of each other.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:twoequivalence}]
 
  We first prove by induction on the rules in \eqref{eq:congr3} that if $\s \dot{\sim} \t$ then $\CatT{Q_{\ThPB}}(\s) \eqsyn \CatT{Q_{\ThPB}}(\t)$.
Consider the case of the rule $(\ThPB)$: in this case $\s=\tapeFunct{c}$, $\t=\tapeFunct{d}$ and $c\eqPB d$. Thus $\CatT{Q_{\ThPB}}(\s)= \CatT{Q_{\ThPB}}(\t)$.
All the other cases trivially follow from the fact that $\CatT{Q_{\ThPB}}$ is a morphism of rig categories: see \cite{bonchi2025tapediagramsmonoidalmonads}.

Again, by induction on the rules, we prove that if $\CatT{Q_{\ThPB}}(\s) \eqsyn \CatT{Q_{\ThPB}}(\t)$ then $\s \dot{\sim} \t$.
Here the only non-trivial cases are $(R)$, $\eqref{ax:AXPBP1}$ and $\eqref{ax:AXPBP2}$. For $(R)$, if $\CatT{Q_{\ThPB}}(\s) = \CatT{Q_{\ThPB}}(\t)$, then by Proposition \ref{prop:quotienttheory}, $\s \tapeeqPB \t$. Hence, $\s \dot{\sim} \t$. For $\eqref{ax:AXPBP1}$, if $\CatT{Q_{\ThPB}}(\s) \overset{\eqref{ax:AXPBP1}}{=} \CatT{Q_{\ThPB}}(\t)$, then $\s$ is $\tapeeqPB$-equivalent to the left hand side of \eqref{ax:AXPBP1} and $\t$ is $\tapeeqPB$-equivalent to the right hand side of \eqref{ax:AXPBP1}. Hence, they are $\dot{\sim}$-equivalent, and applying transitivity of $\dot{\sim}$, we conclude that $\s \dot{\sim} \t$. The case of $\eqref{ax:AXPBP2}$ is analogous.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:bottomstar2}]
 \begin{align}
  \Flipn{\bot}[t]&=\Flip{\bot}[t] ;\ncopierbis[t]  \tag{Def.\ of $\Flipn{\bot}$}\\
  &\sim \Tcounitempty{};\Tunit{}; \ncopierbis[t]  \tag{Axiom \ref{ax:AXPBP2}}\\
  &=  \Tcounitempty{};\Tunitm{n} \tag{\eqref{ax:tapes:cobangnat}}\\
  &= \star_{A^0,A^n}. \tag{Def. of $\star$}
 \end{align}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:PBP2}]
Consider the following derivation: 
\begin{align}
  \frac{1}{2^n} \cdot \t &= \frac{1}{2^n}\cdot (\id{A^n};\t) \notag\\
  &= (\frac{1}{2^n}\cdot \id{A^n});\t \tag{$\Cat{PCA}$-enrichment} \\ 
  &\sim (\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b});\t \tag{Lemma \ref{lemma:axiomsninput}}\\
  &= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b};\t \tag{\eqref{eq:enr}}\\
  &\sim \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b};\s \tag{Hp.}\\
  &=(\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b});\s \tag{\eqref{eq:enr}}\\
  &\sim (\frac{1}{2^n}\cdot \id{A^n});\s \tag{Lemma \ref{lemma:axiomsninput}}\\
  &= \frac{1}{2^n} \cdot \s. \tag{$\Cat{PCA}$-enrichment} 
\end{align}
Hence, applying axiom \eqref{ax:canc}, we conclude that $\t \eqsyn \s$.
\end{proof}

\begin{proof}[proof of Lemma~\ref{lemma:axiomsninput}]
By induction  on $n$. The base case is trivial. For the inductive step, we have
 \begin{align}
  \frac{1}{2^{n+1}}\cdot \id{A^{n+1}}&= \frac{1}{2^n}\frac{1}{2}\cdot( \id{A}\otimes \id{A^n}) \notag\\
  &= \frac{1}{2^n}\cdot\left(\frac{1}{2}\cdot \id{A}\otimes \id{A^n} \right) \tag{\eqref{eq:monoidalenrichment}}\\
  &= (\frac{1}{2}\cdot \id{A})\otimes (\frac{1}{2^n}\cdot \id{A^n}) \tag{\eqref{eq:monoidalenrichment}}\\
  &\sim (\frac{1}{2}\cdot \id{A})\otimes \left(\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b}\right) \tag{Inductive hypothesis}\\
  &\sim (\coflip{1}[t];\Flip{1}[t] +_{\frac{1}{2}} \coflip{0}[t];\Flip{0}[t]) \otimes \left(\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b}\right) \tag{Axiom \ref{ax:AXPBP1}}\\
  &= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\left((\coflip{1}[t];\Flip{1}[t] +_{\frac{1}{2}} \coflip{0}[t];\Flip{0}[t]) \otimes (\overleftarrow{b};\overrightarrow{b})\right) \tag{\eqref{eq:monoidalenrichment}}\\
  &=\sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\left(((\coflip{1}[t];\Flip{1}[t]) \otimes (\overleftarrow{b};\overrightarrow{b})) +_{\frac{1}{2}} ((\coflip{0}[t];\Flip{0}[t]) \otimes (\overleftarrow{b};\overrightarrow{b}))\right) \tag{SMC}\\
  &= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\left((\coflip{1}[t]\otimes \overleftarrow{b});(\Flip{1}[t]\otimes \overrightarrow{b}) +_{\frac{1}{2}} (\coflip{0}[t]\otimes \overleftarrow{b});(\Flip{0}[t]\otimes \overrightarrow{b})\right) \tag{\eqref{eq:monoidalenrichment}}
 \end{align}
 Now, since the set $\{\Flip{1}[t]\otimes \overrightarrow{b}, \Flip{0}[t]\otimes \overrightarrow{b}\}$ as $\overrightarrow{b}\in \Cat{B}[1,A^n]$ is exactly $\Cat{B}[1,A^{n+1}]$, then, rearranging the above sum we obtain $\frac{1}{2^{n+1}}\cdot \id{A^{n+1}}= \sum_{\overrightarrow{b}\in \Cat{B}[1,A^{n+1}]}^{} \frac{1}{2^{n+1}}\cdot\overleftarrow{b};\overrightarrow{b}$, as desired.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lemma:Ffaith}]
  Since $F$ is the composition of an isomorphism with $\stmat{\ParJ_2^\sharp}$ and we have the isomorphism $\stmat{\Cat{Par}_2^+}[A^0,A^m]\cong \Cat{Par}_2^+[A^0,A^m]$, we prove that $\ParJ_2^\sharp\colon\Cat{Par}_2^+
   \to \KlD_2$ is faithful when restricted to $\Sets_2^+[1,2^m]$. Now recall from Theorem~\ref{thm:freeenriched} that $\ParJ_2^\sharp$ is the identity-on-objects functor sending a subdistribution $d\in \Cat{Par}_2^+[1,2^m]$ into the subdistribution $\ParJ_2^\sharp(d)= \sum_{f\in \Cat{Par}_2[1,2^m]} d(f)\cdot{\ParJ_2(f)}$. Hence, if $d\in \Sets_2^+[1,2^m]$, then $\ParJ_2^\sharp(d)= \sum_{f\in \Sets_2[1,2^m]} d(f)\cdot{\ParJ_2(f)}=\sum_{f\in \Sets_2[1,2^m]} d(f)\cdot{\delta_{f(\bullet)}}$, where $f(\bullet)\in 2^m$. Hence, $\ParJ_2^\sharp$ restricted to $\Sets_2^+[1,2^m]$ provides the obvious bijection $$\Dis(\Sets_2[1,2^m])\cong \Dis(2^m) \cong   \KlD_2[1,2^m]\text{.}$$ 
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lemma:PBP0}]
Since $\CatT{\Diag{\ThPB}}\cong \stmat{\Diag{\ThPB}^+}$,  $\t$ corresponds to  a subdistribution on $\Diag{\ThPB}[A^0,A^m]$. By Lemma~\ref{lemma:caratterizzazionecircuiti0n}, each partial Boolean circuit in $\Diag{\ThPB}[A^0,A^m]$ is either a Boolean circuit in $\Diag{\SigB}[1,A^m]$ or it is of the form $\Flipm{\bot}$. Hence, we can rearrange the subdistribution corresponding to $\t$ into a tape of the desired form.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:PBP1}]
  By Lemma~\ref{lemma:PBP0}, we can write 
  \begin{equation}\label{eq:BLABLA}
  \t=(\sum_{i=1}^{n}p_i\cdot b_i)+_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t]) \text{ and }\t'=(\sum_{j=1}^{n'}p'_j\cdot b'_j)+_{p'}(\star_{A^0,A^m} +_{q'} \Flipm{\bot}[t])\end{equation} 
  for some $p_i,p'_j\in (0,1)$, for $i=1,\dots,n$ and $j=1,\dots,n'$, $p,p',q,q'\in [0,1]$  such that $\sum_{i=1}^{n}p_i= 1$ and $\sum_{j=1}^{n'}p'_j= 1$, where $b_i\colon A^0 \to A^m\in \Cat{B}[1,A^m]$ and $b'_j\colon A^0 \to A^m\in \Cat{B}[1,A^m]$. Then,
  \begin{align}
    F(\t)&= F((\sum_{i=1}^{n}p_i\cdot b_i) +_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t])) \tag{\eqref{eq:BLABLA}}\\
    &= F((\sum_{i=1}^{n}p_i\cdot b_i)) +_p(F(\star_{A^0,A^m}) +_q F(\Flipm{\bot}[t])) \tag{$F$ pca-enriched}\\
    &= F((\sum_{i=1}^{n}p_i\cdot b_i)) +_p (\star_{1,2^m} +_q \star_{1,2^m}) \tag{$\ParJ^\sharp(\star_{A^0,A^m})=\star_{1,2^m}=\ParJ^\sharp(\Flipm{\bot})$}\\
    &= p\cdot F(\sum_{i=1}^{n}p_i\cdot b_i) \tag{Idemp.\ in (\ref{eq:pca})}\\
    &=F(p\cdot \sum_{i=1}^{n}p_i\cdot b_i)\tag{$F$ pca-enriched}
  \end{align}
  and similarly $F(\t')=F(p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j)$. Hence, $F(p\cdot \sum_{i=1}^{n}p_i\cdot b_i)=F(p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j)$, and Lemma~\ref{lemma:Ffaith} implies that  
  \begin{equation}\label{BLA2}p\cdot \sum_{i=1}^{n}p_i\cdot b_i=p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j\text{.}\end{equation} Thus,
  \begin{align}
    \t&=(\sum_{i=1}^{n}p_i\cdot b_i) +_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t]) \tag{\eqref{eq:BLABLA}}\\
    &\sim  \sum_{i=1}^{n}p_i\cdot b_i +_p(\star_{A^0,A^m} +_q \star_{A^0,A^m}) \tag{Lemma \ref{lemma:bottomstar2}}\\
    &= \sum_{i=1}^{n}p_i\cdot b_i +_p \star_{A^0,A^m} \tag{Idemp.\ in (\ref{eq:pca})}\\
    &= p\cdot \sum_{i=1}^{n}p_i\cdot b_i\tag{Def. $p\cdot-$}\\
    &= p'\cdot \sum_{j=1}^{n'}p'_j\cdot b'_j \tag{\eqref{BLA2}}\\
    &= \sum_{j=1}^{n'}p'_j\cdot b'_j +_{p'} \star_{A^0,A^m} \tag{Def. $p\cdot-$}\\
    &\sim \sum_{j=1}^{n'}p'_j\cdot b'_j +_{p'}(\star_{A^0,A^m} +_{q'} \star_{A^0,A^m}) \tag{Idemp.\ in (\ref{eq:pca})}\\
    &= \sum_{j=1}^{n'}p'_j\cdot b'_j +_{p'}(\star_{A^0,A^m} +_{q'} \Flipm{\bot}[t]) \tag{Lemma \ref{lemma:bottomstar2}}\\
    &= \t'. \tag{\eqref{eq:BLABLA}}
  \end{align}
\end{proof}



\begin{proof}[Additional details for the proof of Theorem~\ref{thm:completenessPBPtapes}]
    In the main text we have already proved that $H$ is faithful for arrows of type $A^n \to A^m$.
     This fact and convex products easily entail that $H$ is faithful for arrows $\s,\t \colon A^k \to \bigoplus_{i=1}^nA^{m_i}$. 
Indeed, by Theorem~\ref{thm:TCconvexbiproductcategory}, 
\begin{equation}\label{eq:boh}\s=\langle \s_1, \dots, \s_n \rangle_{\vec{q}} \quad \t=\langle \t_1, \dots, \t_n \rangle_{\vec{p}}\end{equation} 
for some $\vec{q}=q_1,\dots, q_n$, $\vec{p}=p_1,\dots, p_n$, $\s_i \colon A^k \to A^{m_i}$ and $\t_i \colon A^k \to A^{m_i}$. Thus
\begin{align*}
H([\s]_\eqsyn) = H([\t]_\eqsyn) & \Rightarrow F(\s)=F(\t) \tag{$F=\eqsynq{Q};H$}\\
& \Rightarrow \text{for all }i \text{, } F(\s);F(\pi_i)=F(\t);F(\pi_i) \\
& \Rightarrow \text{for all }i\text{, } F(\s;\pi_i)=F(\t;\pi_i) \tag{Functoriality} \\
& \Rightarrow  \text{for all }i\text{, }  \s;\pi_i\sim\t;\pi_i \tag{Previous implication}\\
& \Rightarrow  \text{for all }i\text{, }  q_i \cdot \s_i\sim p_i \cdot \t_i \tag{\ref{eq:boh}}\\
& \Rightarrow  \text{for all }i\text{, }  [q_i \cdot \s_i]_\sim = [p_i \cdot \t_i]_\sim 
\end{align*}
%To conclude that $[\s]_\sim=[\t]_\sim$, observe that 
Now \cite[Thm.quoz.??]{arxivprobbooltapes} states that $\CatT{\Diag{\ThPB}}_\sim$ is a convex biproduct category and that the quotient functor $Q_\eqsyn\colon \CatT{\Diag{\ThPB}} \to \CatT{\Diag{\ThPB}}_\sim$ is a morphism of convex biproduct categories.  Hence, Proposition~\ref{prop:functor 1 e mezzo} implies that $(\bigoplus_{i=1}^nA^{m_i}, [\pi_i]_\sim)$ is the $n$-ary convex product of $A^{m_1}, \dots, A^{m_n}$ in $\CatT{\Diag{\ThPB}}_\sim$ and $ [\s]_\sim$ is the unique arrow such that for all $i=1,\dots,n$,
\begin{align}
 [\s]_\sim;[\pi_i]_\sim &= [\s;\pi_i]_\sim \tag{Functoriality of $Q_\eqsyn$}\\
  &=[q_i \cdot \s_i]_\sim \tag{\ref{eq:boh}}\\
 &=q_i\cdot [\s_i]_\sim; \tag{pca-enrichment of $\CatT{\Diag{\ThPB}}_\sim$}
\end{align}
while $[\t]_\sim$ is the unique arrow such that for all $i=1,\dots,n$,
\begin{align}
  [\t]_\sim;[\pi_i]_\sim&= [\t;\pi_i]_\sim \tag{Functoriality of $Q_\eqsyn$}\\
  &= [p_i \cdot \t_i]_\sim \tag{\ref{eq:boh}}\\
  &=p_i\cdot [\t_i]_\sim. \tag{pca-enrichment of $\CatT{\Diag{\ThPB}}_\sim$}
\end{align}
Hence, since for all $i=1,\dots,n$, $[q_i \cdot \s_i]_\sim = [p_i \cdot \t_i]_\sim$, we have $[\s]_\sim = [\t]_\sim$.

%$[\s]_\sim=\langle [\s_1]_\sim, \dots, [\s_n]_\sim \rangle_{\vec{q}}$ and $[\t]_\sim=\langle [\t_1]_\sim, \dots, [\t_n]_\sim \rangle_{\vec{p}}$. Since for all $i$, $[\t];[\pi_i]_\sim$ and  $[\s];[\pi_i]_\sim$ are both equal to  $p_i\cdot[\t_i]_\sim=[p_i \cdot \t_i]_\sim=[q_i \cdot \s_i]_\sim$, the universal  property of  n-ary convex products in $\CatT{\Diag{\ThPB}}_\sim$ implies that $[\s]_\sim=[\t]_\sim $.

For arrows of arbitrary type $\bigoplus_{j=1}^o A^{k_j} \to \bigoplus_{i=1}^nA^{m_i}$, one can easily rely on the universal property of coproducts and the case that we just proved.
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:completenessPBPtapes}]
By Theorem~\ref{thm:completenessPBPtapes}, $H$ is faithful. Since $I$ is exactly $H;G$ and $G$ is faithful by Theorem~\ref{thm:matfree}, then $I$ is also faithful. The following derivation concludes the proof.
  \begin{align}
    \dsem{\s}=\dsem{\t} &\Longleftrightarrow (\CatT{Q_{\ThPB}}; Q_\eqsyn ; I) (\s)= (\CatT{Q_{\ThPB}}; Q_\eqsyn ; I) (\t) \tag{$\dsem{-}= \CatT{Q_{\ThPB}}; Q_\eqsyn ; I$}\\
    &\implies   (\CatT{Q_{\ThPB}}; Q_\eqsyn ) (\s)= (\CatT{Q_{\ThPB}}; Q_\eqsyn )(\t) \tag{$I$ is faithful} \\
    &\Longleftrightarrow \CatT{Q_{\ThPB}}  (\s) \eqsyn \CatT{Q_{\ThPB}}(\t) \tag{Def. $Q_\eqsyn$}\\
    &\Longleftrightarrow \s \dot{\sim} \t \tag{Proposition \ref{prop:twoequivalence}}
  \end{align}
\end{proof}





==> sections/probabilisticbooleancircuits-NEW.tex <==

\section{Probabilistic Boolean Circuits}\label{sec:probboolcircuits}

%In this section we recall the definition of probabilistic Boolean circuits from \cite{piedeleu2025boolean}. To do that, we first deal with Boolean circuits in Section~\ref{ssec:boolean}, then we introduce  partial Boolean circuits in Section~\ref{ssec:partialboolean} and provide a complete axiomatisation. Finally, in Section~\ref{ssec:probabilisticboolean} we introduce probabilistic Boolean circuits  and their semantics.

Before proceeding, recall that a \emph{monoidal signature} is a tuple $(\sort, \sign, \ari, \coar)$ where $\sort$ is a set of basic sorts, hereafter denoted by $A,B,\dots$, $\sign$ is a set of generators, denoted by $s,t, \dots$, and $\ari,\coar \colon \sign \to \sort^*$ assign to each symbol its arity and coarity, i.e., words over $\sort$, denoted by $U,V,W$. We consider terms generated by the following grammar, where $A,B \in \sort$ and $s \in \Sigma$:
\begin{equation}\label{stringdiagramGrammar}
\setlength{\arraycolsep}{3pt} % spaziatura orizzontale
%\renewcommand{\arraystretch}{1.1} % opzionale: un po' di respiro verticale
\begin{array}{rcccccccccccccccc}
c & ::= & \id{A} & \mid & \id{\uno} & \mid & \gen & \mid & \symmt{A}{B} & \mid & c ; c & \mid & c \per c
\end{array}
\end{equation}
These terms can be typed according to the rules in Table~\ref{fig:freestricmmoncatax}. Well-typed terms $c \colon U \to V$, taken modulo the axioms in the same table, correspond to the arrows of a strict symmetric monoidal category $(\DiagS, \per, \uno)$, namely the one freely generated by $\sign$.
Arrows of $\DiagS$ admit a graphical representation in terms of \emph{string diagrams} \cite{joyal1991geometry,selinger2010survey}. The grammar above can be depicted diagrammatically as follows:
\begin{equation*}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{rc c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c}
        $c$  & $\Coloneqq$ &  $\wire{A}$ & $ \tikzfig{empty} $ & $ \Cgen{\gen}{A}{B} $ & $ \Csymm{A}{B} $ & $ \tikzfig{seq_compC} $ & $ \tikzfig{par_compC}$ \\
    \end{tabular}
\end{equation*}
The diagrammatic notation internalises the axioms in Table~\ref{fig:freestricmmoncatax}, yielding proofs that are both more concise and more intuitive. Throughout the paper, we will also rely on the term-based notation, which is often more convenient for inductive definitions.

A \emph{monoidal theory} $\mathbb{T}=(\sign, E)$ consists of a monoidal signature equipped with a set $E$ of pairs of arrows of $\DiagS$ of the same type. Let $=_{\mathbb{T}}$ be an equivalence relation on arrows  of $\DiagS$ obtained as the congruence closure (w.r.t. $;$ and $\otimes$) of $E$. We write $\DiagT$ for the monoidal category obtained as the quotient of $\DiagS$ by $=_{\mathbb{T}}$ and $Q_{\mathbb{T}}\colon \Diag{ \sign} \to \Diag{\mathbb{T}}$ for the monoidal functor mapping each diagram into its $=_{\mathbb{T}}$ equivalence class.


\begin{table}[H]
\resizebox{\textwidth}{!}{%
$
\begin{array}{c}
\toprule
\begin{array}{c}
    \begin{array}{ccccc}
        {\sigma_{A, B}^{\per} \colon A \per B \to B \per A} 
    \end{array}    
\\[0.3em]
    \begin{array}{ccccc}
        {id_\uno \colon \uno \to \uno} &
        {id_A \colon A \to A} &
        \inferrule{\ari(\gen)=U \quad \coar(\gen)= V}{\gen \colon U \to V} &
        \inferrule{c \colon U \to V \and d \colon V \to W}{c ; d \colon U \to W} &
        \inferrule{c \colon U_1 \to V_1 \and d \colon U_2 \to V_2}{c \per d\colon U_1 \per U_2 \to V_1 \per V_2}       
    \end{array}
\end{array}
\\[0.5em]
\begin{array}{cc}
\midrule
\begin{array}{c}
(c;d);e=c;(d;e) \qquad id_U;c=c=c;id_Q\\
(c_1\per c_2) ; (d_1 \per d_2) = (c_1;d_1) \per (c_2;d_2)
\end{array} 
&
\begin{array}{c}
id_{\uno}\per c = c = c \per id_{\uno} \qquad (c \per d)\, \per e = c \per \,(d \per e) \\
\sigma_{U, V}; \sigma_{V, U}= id_{U \per V} \qquad (\gen \per id_W) ; \sigma_{V, W} = \sigma_{U,W} ; (id_W \per \gen)
\end{array}
\end{array}\\
\bottomrule
\end{array}
$
}
\caption{Typing rules (top) and axioms (bottom) for freely generated strict symmetric monoidal categories.}
\label{fig:freestricmmoncatax}
\end{table}






Consider monoidal signatures with a single sort, $\sort = \{A\}$, and sets of generators
\[
\SigB \defeq \{\Andgate, \Notgate, \Flip{1}, \CBcopier, \CBdischarger\}, \quad
\SigPB \defeq \SigB \cup \{\CBcocopier\}, \quad
\SigPRB \defeq \SigPB \cup \{ \Flip{p} \mid p \in (0,1)\}.
\]
Arities and coarities are determined by the number of input and output ports. For instance, $\Andgate$ has arity $A^2 = AA$ and coarity $A$, while $\CBdischarger$ has arity $A$ and coarity $A^0 = 1$. Since $\sort = \{A\}$, the objects of the categories $\Diag{\SigB}$, $\Diag{\SigPB}$, and $\Diag{\SigPRB}$ are words of the form $A^n$ for some $n \in \mathbb{N}$.

Diagrams in $\Diag{\SigB}$ are Boolean circuits; those in $\Diag{\SigPB}$  partial Boolean circuits; and those in $\Diag{\SigPRB}$  probabilistic Boolean circuits. %There are evident embeddings
%\[
%\xymatrix{\Diag{\SigB} \ar@{^{(}->}[r] & \Diag{\SigPB}}
%\qquad
%\xymatrix{\Diag{\SigPB} \ar@{^{(}->}[r] & \Diag{\SigPRB}}.
%\]
Our main focus is $\Diag{\SigPRB}$, although it will be convenient to also consider its fragments $\Diag{\SigPB}$ and $\Diag{\SigB}$.

The first three generators of $\SigB$ correspond to the operations and constants of Boolean algebras, namely $\wedge$, $\neg$, and $1$. The generator \emph{copy}, denoted by $\CBcopier$, takes a Boolean signal as input and produces two identical outputs. The generator \emph{discard}, denoted by $\CBdischarger$, takes a Boolean signal as input and discards it.

The generator $\CBcocopier$ in $\SigPB$ can be understood as the dual of $\CBcopier$: it compares two input signals and, if they are equal, returns that value; otherwise, it produces no output.
Finally, $\Flip{p}$ denotes a probabilistic gate with no inputs that outputs a Boolean signal, equal to $1$ with probability $p$ and to $0$ with probability $1-p$.

\medskip


To formally define the semantics, it is convenient to recall now some key notions. We write $\Dis(X)$ for the set of all (finitely supported probability) \emph{subdistribution} over a set  $X$, namely, functions $d\colon X\to [0,1]$  such that $\sum_{x\in X}d(x)\leq 1$, and $d(x)\neq 0$ for  finitely many $x\in X$. For all $x\in X$, we write $\delta_x \in \Dis(X)$ for the Dirac distribution; $\star\in \Dis(X)$ for the null subdistribution: $\star(x)=0$ for all $x\in X$; for all $p\in (0,1)$ and $d_1,d_2\in \Dis(X)$, we write $d_1+_pd_2$ for the subdistributions mapping each $x\in X$ into $p\cdot d_1(x) + (1-p)\cdot d_2(x)$.

The assignment $X\mapsto \Dis(X)$ extends to a functor $\subdistr\colon \Sets \to \Sets$ which carries the structure of a monad (see e.g.,~\cite{hasuo2007generic}). We consider, the Kleisli category of such monad, hereafter denoted by $\KlD$. 
Objects of $\KlD$ are sets; morphisms \(f \colon X \to Y\) are functions \(X \to \subdistr(Y)\). 
  We often write \(f(y \mid x)\) for \(f(x)(y)\), as this number represents the probability that \(f\) returns \(y\) given the input \(x\).
  Identities \(\id{X} \colon X \to \subdistr(X)\) map each element \(x \in X\) to \(\delta_{x}\).
  For two functions \(f \colon X \to \subdistr(Y)\) and \(g \colon Y \to \subdistr(Z)\), their composition in $\KlD$ is defined as \(f ; g (z \mid x) \defeq \sum_{y \in Y} f(y \mid x) \cdot g(z \mid y)\).

This categories carries a symmetic monoidal structure
$(\KlD, \otimes, \uno)$, where $\otimes$ is the cartesian product of sets with unit the singleton $\uno \defeq \{\bullet\}$ and, for arrows  \(f \colon X \to Y\) and \(g \colon X' \to Y'\), $f\per g\colon X\otimes X' \to Y \otimes Y'$ is defined, for all $x\in X$, $x'\in X'$, $y\in Y$, $y'\in Y'$, as follows.
\begin{equation}\label{ex:products}
\begin{aligned}
f \per g(y,y' \mid x,x') &\defeq f(y \mid x) \cdot g(y' \mid x')
\end{aligned}
\end{equation}
For all sets $X,Y$, symmetries $\symmt{X}{Y}\colon X \otimes Y \to Y \otimes X$ are given as $\symmt{X}{Y}((x,y)|(y',x')) \defeq 1$ if $x=x'$ and $y=y'$ and $\symmt{X}{Y}((x,y)|(y',x')) \defeq 0$ otherwise.


%\[
%    \begin{array}{rclrclrcl}
%      \osem{\Andgate}(z|(x,y)) & \defeq &  \begin{cases}1 &\text{if }z=x\wedge y\\ 0 & \text{else}\end{cases}
%      &
%      \osem{\Notgate}(y|x) & \defeq &  \begin{cases}1 &\text{if }y= \neg x \\ 0 & \text{else}\end{cases}
%      & 
%      \osem{\Flip{1}}(x|\bullet)  & \defeq &  \begin{cases}1 &\text{if }x=1 \\ 0 & \text{else}\end{cases}
%\\[4pt]
%       \osem{\CBcopier}((z,y)|x) & \defeq &  \begin{cases}1 &\text{if }z=y=x\\ 0 & \text{else}\end{cases}  & \osem{\CBdischarger}(\bullet | x) & \defeq & 1 & \osem{\CBcocopier}(z|(x,y)) & \defeq &  \begin{cases}1 &\text{if }z=y=x\\ 0 & \text{else}\end{cases} \\
%          \end{array}
%  \]

\medskip

The semantics is defined by first interpreting each generator  $s\in \SigPRB$ with arity $A^n$ and coarity $A^m$ into a $\KlD$-arrow $\osem{s} \colon 2^n \to 2^m$ where $2$ is the set of Booleans $\{0,1\}$.
For all booleans $x,y\in 2$, these arrows are defined as follows. 
\begin{equation}\label{eq:semanticsFlip}
{\small    
\begin{array}{cc}\begin{array}{rclrclrclrcl}
      \osem{\Andgate}\colon 2 \times 2& \to & 2  & \osem{\Notgate}\colon  2& \to & 2 & \osem{\Flip{1}} \colon 1 & \to & 2&  \osem{\Flip{p}}\colon 1& \to & 2  \\
      (x,y)&\mapsto&\delta_{x\wedge y} &  x & \mapsto & \delta_{\neg x} & \bullet &\mapsto&\delta_{1} &  \bullet&\mapsto& \delta_1 +_p \delta_0 \\
      \end{array}
      \\[4pt]
      \\[4pt]
      \begin{array}{rclrclrcl}
       \osem{\CBcopier} \colon 2  & \to & 2\times 2 & \osem{\CBdischarger} \colon 2 & \to & 1 & \osem{\CBcocopier} \colon 2 \times 2 & \to & 2  \\
      x &\mapsto&\delta_{(x,x)} & x &\mapsto&\delta_{\bullet} & (x,y) &\mapsto& \begin{cases}\delta_{x} &\text{if }x=y\\ \star & \text{else}\end{cases}, 
    \end{array}
    \end{array}}
  \end{equation}
Then, the semantics of diagrams in $\Diag{\SigPRB}$ is defined by extending inductively the above interpretation by means of the symmetric monoidal structure of $(\KlD,\per, \uno)$:
\begin{equation}\label{eq:smfunctor}
\begin{array}{ccccc}
\osem{\id{A}}\defeq \id{2} &   \osem{\id{\uno}}\defeq \id{1} &  \osem{\symmt{A}{A}}\defeq \symmt{2}{2}
 & \osem{ c ; d }\defeq \osem{c} ; \osem{d} & \osem{c \per d} = \osem{c} \per \osem{d}
\end{array}
\end{equation}
Crucially, \eqref{eq:semanticsFlip} and \eqref{eq:smfunctor} defines a symmetric monoidal functor $\osem{-}\colon \Diag{\SigPRB} \to \KlD$ defined on objects as  $\osem{A^n} = 2^n$.


The reader can easily see that the functor $\osem{-}$ restricted to $\Diag{\SigB}$ corestricts to $\Sets$. Similarly  $\osem{-}$ restricted to $\Diag{\SigPB}$ corestrict to $\Cat{Par}$, the category of sets and partial functions.
Intuitively these facts mean that all boolean circuits denote functions, while partial boolean circuits denote partial functions. Formally, there exists symmetric monoidal functor $\osemB{-}\colon \Diag{\SigB} \to \Sets$ and $\osemPB{-}\colon \Diag{\SigPB} \to \Cat{Par}$ making the following diagram commutes
\[
\xymatrix{\Diag{\SigB} \ar@{^{(}->}[r] \ar[d]_{\osemB{-}}& \Diag{\SigPB} \ar@{^{(}->}[r] \ar[d]|{\osemPB{-}} & \Diag{\SigPRB} \ar[d]^{\osem{-}}\\
\Sets \ar@{^{(}->}[r]_{\Pa}& \Cat{Par} \ar@{^{(}->}[r]_{\ParJ}& \KlD
}
\]
where the horizontal arrows are the obvious embeddings. For later use, it is important to illustrate $\ParJ\colon \Cat{Par} \to \KlD$: it is the identity on objects and associates to a partial function $f\colon X \to Y$ the function $\ParJ(f)\colon X \to \Dis(Y)$, mapping $x$ to $\delta_{f(x)}$, if $f(x)$ is defined and to the null distribution $\star$ otherwise. 







\medskip
Figures~4 and~5 in \cite{piedeleu2025boolean} provide a sound and complete equational axiomatisation of probabilistic Boolean circuits. The system essentially consists of the axioms of Boolean algebras (reported in Figure~\ref{tab:booleanalgebra}), together with four non-trivial axioms governing the behaviour of $\Flip{p}$ and additional axioms for $\CBcocopier$, which differ from those presented in Figure~\ref{tab:partialbooleanalgebra}.

Importantly, the equivalence induced by these axioms is strictly coarser than the one given by $\osem{-}$. In fact, two diagrams $c$ and $d$ are equivalent under the axioms of \cite{piedeleu2025boolean} if and only if $\osem{c} \propto \osem{d}$. The relation $\propto$ is defined on arrows of $\KlD$ by setting $f \propto g$ whenever there exists a real number $\lambda > 0$ such that $f(y\mid x) = \lambda \cdot g(y\mid x)$ for all $x \in X$ and $y \in Y$. %In the next section, we provide a complete  axiomatisation for the equivalence induced by $\osem{-}$ by means of probabilistic tape diagrams.








Formally, the semantics of these diagrams is given by the monoidal functor  $\osemB{-}\colon \Diag{{\SigB}} \to \Sets$ defined on objects as $A^n \mapsto 2^n$ where $2$ is the set of Booleans  $\{0,1\}$; for arrows it is defined by first interpreting the generators as functions in $\Sets$
  \[
    \begin{array}{rclrclrcl}
      \osemB{\Andgate}\colon 2 \times 2& \to & 2  & \osemB{\Notgate}\colon  2& \to & 2 & \osemB{\Flip{1}} \colon 1 & \to & 2 \\
      (x,y)&\mapsto& x\wedge y &  x & \mapsto & \neg x & \bullet &\mapsto&1\\[4pt]
       \osemB{\CBcopier} \colon 2  & \to & 2\times 2 & \osemB{\CBdischarger} \colon 2 & \to & 1 & %\osemB{\Flip{p}} \colon 1 & \to & 2  
       \\
      x &\mapsto&(x,x) & x &\mapsto&{\bullet} & %\bullet &\mapsto& \delta_1 +_p \delta_0
    \end{array}
  \]
and then inductively by means of the structure of the monoidal category $(\Sets, \otimes ,\uno)$: for instance, $\osemB{c_1\otimes c_2}=\osemB{c_1}\otimes \osemB{c_2}$ where the second $\otimes$ is the standard cartesian product of functions. 

The monoidal theory $\ThB$ consists of the signature $\SigB$ together with the axioms listed in Figure~\ref{tab:booleanalgebra}. 
The equalities in the first block are the standard axioms of Boolean algebras. 
The constant $\Flip{0}$ and the $\Orgate$ gate are defined as expected (see Figure~\ref{table:multiplexer}). 
Note that, in the string-diagrammatic setting, the structural maps $\CBcopier$ and $\CBdischarger$ must be made explicit.
The equalities in the second block state that $\CBcopier$ and $\CBdischarger$ form a commutative comonoid. 
The equalities in the third and fourth blocks impose naturality of $\CBcopier$ and $\CBdischarger$, respectively.


The congruence with respect to $;$ and $\otimes$ generated by the axioms in Figure~\ref{tab:booleanalgebra} is denoted by $\eqB$. 
We write $\Diag{\ThB}$ for the quotient of $\Diag{\SigB}$ by $\eqB$.

As expected, the equalities in Figure~\ref{tab:booleanalgebra} provide a sound and complete axiomatization of the equality induced by $\osemB{-}$. See e.g. \cite[Theorem 3.2]{piedeleu2025boolean}.

\begin{theorem}\label{thm:completenessbooleancircuits}
For all  $c,d\in \Diag{\SigB}$, $\osemB{c}=\osemB{d}$ iff $c\eqB d$.
\end{theorem}


\begin{figure}
  \scalebox{0.8}{%
  \begin{tabular}{ccccc}

  % =====================
  % ---- B axioms ----
  % =====================

  \mylabelbis{ax:B1}{B1}%
  $\tikzfig{tapes/cipriano/axB1left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B1}}{=}$\,}\tikzfig{tapes/cipriano/axB1right}$
  & &
  \mylabelbis{ax:B2l}{B2l}\mylabelbis{ax:B2r}{B2r}%
  $\tikzfig{tapes/cipriano/axB2left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B2l}}{=}$\,}\tikzfig{tapes/cipriano/axB2middle}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B2r}}{=}$\,}\tikzfig{tapes/cipriano/axB2right}$
  & &
  \mylabelbis{ax:B3}{B3}%
  $\tikzfig{tapes/cipriano/axB3left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B3}}{=}$\,}\tikzfig{tapes/cipriano/axB3right}$
  \\

  \mylabelbis{ax:B4}{B4}%
  $\tikzfig{tapes/cipriano/axB4left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B4}}{=}$\,}\tikzfig{tapes/cipriano/axB4right}$
  & &
  \mylabelbis{ax:B5}{B5}%
  $\tikzfig{tapes/cipriano/axB5left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B5}}{=}$\,}\tikzfig{tapes/cipriano/axB5right}$
  & &
  \mylabelbis{ax:B6}{B6}%
  $\tikzfig{tapes/cipriano/axB6left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B6}}{=}$\,}\tikzfig{tapes/cipriano/axB6right}$
  \\

  & &
  \mylabelbis{ax:B7}{B7}%
  $\tikzfig{tapes/cipriano/axB7left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B7}}{=}$\,}\tikzfig{tapes/cipriano/axB7right}$
  & &
  \\

  \midrule

  % =====================
  % ---- A axioms ----
  % =====================

  \mylabelbis{ax:A1}{B8}%
  $\tikzfig{tapes/cipriano/axA1left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A1}}{=}$\,}\tikzfig{tapes/cipriano/axA1right}$
  & &
  \mylabelbis{ax:A2l}{B9l}\mylabelbis{ax:A2r}{B9r}%
  $\tikzfig{tapes/cipriano/axA2left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A2l}}{=}$\,}\tikzfig{tapes/cipriano/axA2middle}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A2r}}{=}$\,}\tikzfig{tapes/cipriano/axA2right}$
  & &
  \mylabelbis{ax:A3}{B10}%
  $\tikzfig{tapes/cipriano/axA3left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A3}}{=}$\,}\tikzfig{tapes/cipriano/axA3right}$
  \\

  \midrule

  % =====================
  % ---- C axioms ----
  % =====================

  \mylabelbis{ax:C1}{B11}%
  $\tikzfig{tapes/cipriano/axC1left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:C1}}{=}$\,}\tikzfig{tapes/cipriano/axC1right}$
  & &
  \mylabelbis{ax:C2}{B12}%
  $\tikzfig{tapes/cipriano/axC2left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:C2}}{=}$\,}\tikzfig{tapes/cipriano/axC2right}$
  & &
  \mylabelbis{ax:C3}{B13}%
  $\tikzfig{tapes/cipriano/axC3left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:C3}}{=}$\,}\tikzfig{tapes/cipriano/axC3right}$
  \\

  \midrule

  % =====================
  % ---- D axioms ----
  % =====================

  \mylabelbis{ax:D1}{B14}%
  $\tikzfig{tapes/cipriano/axD1left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:D1}}{=}$\,}\tikzfig{tapes/cipriano/axD1right}$
  & &
  \mylabelbis{ax:D2}{B15}%
  $\tikzfig{tapes/cipriano/axD2left}\raisebox{-0.6ex}{$\stackrel{\eqref{ax:D2}}{=}$}\tikzfig{tapes/cipriano/axD2right}$
  & &
  \mylabelbis{ax:D3}{B16}%
  $\tikzfig{tapes/cipriano/axD3left}\raisebox{-0.6ex}{$\stackrel{\eqref{ax:D3}}{=}$}
  \raisebox{-0.5em}{\tikzfig{empty}}$
  \\

  \end{tabular}}%
  \caption{The monoidal theory of Boolean algebras.}
  \label{tab:booleanalgebra}
\end{figure}
Moreover, one can characterise exactly the image of $\Diag{\SigB}$ through $\osemB{-}$. Let $\Sets_2$ be the full subcategory of sets where objects are powers of the set $2$, i.e.,  $2^n$ for all $n \in \mathbb{N}$.


\begin{proposition}\label{prop:foolboolean}
The monoidal functor  $\osemB{-}\colon \Diag{{\SigB}} \to \Sets$ factors as
\[\xymatrix{ \Diag{\SigB} \ar@{->>}[r]& \Diag{\ThB} \ar[r]^{\cong}& \Sets_2 \ar@{^{(}->}[r]& \Sets }\]
where the leftmost and rightmost functor are the obvious quotients and injections and the central arrows is a monoidal isomorphism.
\end{proposition}
\begin{proof}
Faithfulness of the central functor is a direct consequence of Theorem~\ref{thm:completenessbooleancircuits}. Fullness follows from the fact that every function $f\colon 2^n \to 2^m$ corresponds to a vector of $m$ Boolean formulas in $n$ variables, which can be easily encoded as a string diagram in $\Diag{\ThB}$ using Boolean operators, $\CBcopier$ and $\CBdischarger$.
\end{proof}



We conclude this section by fixing some syntactic sugar, collected in Figure~\ref{table:multiplexer}. 
The \emph{xnor} gate $\xnor$  takes two Boolean inputs and outputs $1$ if they are equal and $0$ otherwise. 
The \emph{multiplexer} $\tikzfig{tapes/cipriano/multi}$ takes three inputs and returns one output: if the first input is $1$, then it outputs the second input, otherwise the third input. 
The $m$-ary multiplexer $\Ifgatem$ works similarly, but it takes $2m+1$ inputs: if the first input is $1$, then it outputs the first $m$ inputs, otherwise it outputs the second $m$ inputs. 
Figure~\ref{table:multiplexer} also defines $m$-ary discard $\CBdischargerm$ and copier $\mcopier$. Note that, for the sake of readability of string diagrams, we label wires by  some natural number $n$ as an abbreviation for $A^n$.

\begin{lemma}\label{lemma:multiplexer}
 Let $c$ be a diagram in $\Diag{\SigB}[n,m]$. The following derived laws hold:

\mylabelbis{ax:M1}{D1}
\mylabelbis{ax:M2}{D2}
\mylabelbis{ax:M3}{D3}
\mylabelbis{ax:N1}{D4}
\mylabelbis{ax:N2}{D5}

\[
\begin{array}{c@{\qquad}c@{\qquad}c}

\raisebox{-0.3em}{\tikzfig{tapes/cipriano/D1left}} 
\stackrel{\eqref{ax:M1}}{\eqB}
\tikzfig{tapes/cipriano/D1right}

&
\raisebox{-0.3em}{\tikzfig{tapes/cipriano/D2left}}
\stackrel{\eqref{ax:M2}}{\eqB}
\tikzfig{tapes/cipriano/D2right}

&
\raisebox{-0.3em}{\tikzfig{tapes/cipriano/D3left}}
\stackrel{\eqref{ax:M3}}{\eqB}
\tikzfig{tapes/cipriano/D3right}

\\[1em]

\tikzfig{tapes/cipriano/D4left}
\stackrel{\eqref{ax:N1}}{\eqB}
\tikzfig{tapes/cipriano/D4right}

&
\tikzfig{tapes/cipriano/D5left}
\stackrel{\eqref{ax:N2}}{\eqB}
\tikzfig{tapes/cipriano/D5right}

&

\end{array}
\]
\end{lemma}




\begin{figure}[t]
\centering
\resizebox{0.96\linewidth}{!}{%
\begin{tabular}{@{}l@{}}

% ---- Row 1 ----
$\Orgate \defeq (\Notgate \otimes \Notgate); \Andgate; \Notgate 
\qquad 
\Flip{0} \defeq \Flip{1}; \Notgate
\qquad
\tikzfig{tapes/cipriano/multi} 
\defeq 
\tikzfig{tapes/cipriano/multiexpl}$ \\[4pt]

% ---- Row 2 ----
$\tikzfig{tapes/cipriano/xnorgate}
\qquad
\raisebox{-1em}{\tikzfig{tapes/cipriano/ncopierzero}} 
\raisebox{-0.5em}{$\defeq$}
\raisebox{-0.5em}{\tikzfig{empty}}
\qquad 
\raisebox{-1em}{\tikzfig{tapes/cipriano/ncopier}}$ \\[6pt]

% ---- Row 3 ----
$\raisebox{-1.2em}{\tikzfig{tapes/cipriano/mmultiplexerleftzero}} 
\defeq 
\tikzfig{tapes/cipriano/mmultiplexerrightzero}
\qquad 
\raisebox{-1.2em}{\tikzfig{tapes/cipriano/mmultiplexerleft}} 
\defeq 
\tikzfig{tapes/cipriano/mmultiplexerright}$ \\[6pt]

% ---- Row 4 ----
$\mFlip{1}{0} \defeq \tikzfig{empty}
\qquad
\mFlip{1}{m+1} \defeq \Flip{1} \otimes \mFlip{1}{m}
\qquad
\mCBdischarger{0} \defeq \tikzfig{empty}
\qquad
\mCBdischarger{m+1} \defeq \CBdischarger\otimes \mCBdischarger{m}$

\end{tabular}
}
\caption{Definitions of OR gate, $\Flip{0}$ and multiplexer (top); definitions of XNOR gate and inductive definition of $n$-ary copier (middle); inductive definitions of $m$-ary multiplexer (third row); definitions of $\Flipzero{1}$, $\Flipm{1}$ and $n$-ary dischargers (bottom).}
\label{table:multiplexer}
\end{figure}

%
%
% SUBSECTION
%
%
\subsection{Partial Boolean Circuits}\label{ssec:partialboolean}
Now consider the monoidal signature obtained by adding to $\SigB$ the generator \emph{cocopy} $\CBcocopier$ of arity $A^2$ and coarity $A$. 
\[ PB\defeq \SigB \cup\{\CBcocopier\}\text{}\] 
Intuitively, $\CBcocopier$ is the dual of $\CBcopier$: it compares two inputs and, if these are equal, it outputs that value; otherwise, it produces no output. Thus, string diagrams in $\Diag{PB}$ represent \emph{partial} Boolean functions. 

To formally define their semantics, let us first fix $(\Cat{Par}, \otimes, 1)$ to be the symmetric monoidal category of sets and partial functions, where the monoidal product $\otimes$ is the cartesian product of sets and, for all partial functions $f_1\colon X_1 \to Y_1$ and $f_2\colon X_2 \to Y_2$, $f_1\otimes f_2 \colon X_1 \times X_2 \to Y_1 \times Y_2$ is defined as
\begin{equation}\label{eq:productpar}
f_1\otimes f_2 (x_1,x_2) \defeq \begin{cases} (\,f_1(x_1), \, f_2(x_2)\,) & \text{ if }f_1(x_1)\neq \bot\text{, } f_2(x_2)\neq \bot \\
 \bot & \text{ otherwise}\end{cases}
\end{equation}
for all $(x_1,x_2)\in X_1\times X_2$. Above, and in the rest of the paper, we write $f(x)=\bot$ to say that a partial function $f\colon X \to Y$ is undefined for some $x\in X$. 
One can readily check that the obvious injection $\Pa\colon \Sets \to \Cat{Par}$ is a symmetric monoidal functor.


Now, the semantics of diagrams in $\Diag{PB}$ is given by the monoidal functor $\osemPB{-}\colon \Diag{PB} \to \Cat{Par}$ defined on objects as $A^n \mapsto 2^n$, like $\osemB{-}$; 
for arrows it is defined by first interpreting generators $c \in \SigB$ as $\osemPB{c}\defeq \Pa(\osemB{c})$, the generator $\CBcocopier $ as
  \begin{equation}\label{eq:semcocopier}
    \begin{array}{rcl}
      \osemPB{\CBcocopier}\colon 2 \times 2& \to & 2   \\
      (x,y)&\mapsto& \begin{cases} x &\text{if } x=y\\ \bot & \text{else}\end{cases}    \end{array}
  \end{equation}
and then inductively by means of the structure of the monoidal category $(\Cat{Par}, \otimes ,\uno)$: for instance $\osemB{c_1\otimes c_2}=\osemB{c_1}\otimes \osemB{c_2}$ where the second $\otimes$ is the one in \eqref{eq:productpar}. %A simple inductive argument confirms that $\osemPB{-}$ is an extension of $\osemB{-}$, i.e., the following diagram commutes
%\[
%\xymatrix{\Diag{PB} \ar[r]^{\osemPB{-}} & \Cat{Par}\\ 
%\Diag{B} \ar[r]_{\osemB{-}} \ar@{>->}[u] & \Sets \ar@{>->}[u]_P
%}
%\]
For example, the semantics of the following diagrams
\begin{equation}\label{def:bottom}
  \raisebox{0cm}{\tikzfig{tapes/cipriano/defcoflip}}
\end{equation}
is illustrated below.
  \[
    \begin{array}{rclrclrcl}
      \osemPB{\coflip{1} }\colon 2 & \to & 1  & \osemPB{\coflip{0} }\colon 2 & \to & 1 & \osemPB{\Flip{\bot}}\colon 1 & \to & 2 \\
      x&\mapsto& \begin{cases} \bullet &\text{if } x=1\\ \bot & \text{else}\end{cases}    
      &
      x&\mapsto& \begin{cases} \bullet &\text{if } x=0\\ \bot & \text{else}\end{cases}    
      &
      \bullet &\mapsto & \bot     
      \end{array}
  \]






In this section, we present a complete axiomatization of the equality induced by $\osemPB{-}$, which, to the best of our knowledge, has not been previously established.
The axioms are illustrated in Figure~\ref{tab:partialbooleanalgebra}: the equalities in the first row assert that $\CBcocopier$ is associative, commutative and idempotent; in the second row, there are the usual Frobenius equalities ruling the interaction of $\CBcocopier$ with $\CBcopier$; the two axioms in the third row are more peculiar: the rightmost states that $x\wedge y = 1$ iff $x=y=1$; the leftmost provides a decomposition of  $\CBcocopier$ in terms of $\Andgate$, $\coflip{1}$ and the xnor gate \tikzfig{tapes/cipriano/xnorgatealone}.



%%%%%%%NUOVA TABELLA CON TAG%%%%%%%%%%
\begin{figure}
\centering
\scalebox{0.8}{
{
\setlength{\tabcolsep}{12pt}      % spazio orizzontale
\setlength{\extrarowheight}{9pt}  % spazio verticale aggiuntivo
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{ccc}

% Prima riga
\hspace{1.5em}%
\mylabelbis{ax:F1}{P1}%
$\tikzfig{tapes/cipriano/axF1left}
 \raisebox{-0.6em}{\,\,$\stackrel{\eqref{ax:F1}}{=}$\,\,}
 \tikzfig{tapes/cipriano/axF1right}$
&
\hspace{1.5em}%
\mylabelbis{ax:F2}{P2}%
$\tikzfig{tapes/cipriano/axF2left}
 \raisebox{-0.6em}{\,$\stackrel{\eqref{ax:F2}}{=}$\,}
 \tikzfig{tapes/cipriano/axF2right}$
&
\hspace{1.5em}%
\mylabelbis{ax:F3}{P3}%
$\tikzfig{tapes/cipriano/axF3left}
 \raisebox{-0.6em}{\,\,$\stackrel{\eqref{ax:F3}}{=}$\,\,}
 \tikzfig{tapes/cipriano/axF3right}$
\\[1.2em]

% Seconda riga
\multicolumn{3}{c}{%
  \scalebox{0.85}{%
    \mylabelbis{ax:F4}{P4}%
    \mylabelbis{ax:F5}{P5}%
    $\tikzfig{tapes/cipriano/axF4left}
      \,\stackrel{\eqref{ax:F4}}{=}\,
      \tikzfig{tapes/cipriano/axF4right}
      \,\stackrel{\eqref{ax:F5}}{=}\,
      \tikzfig{tapes/cipriano/axF5}$%
  }%
  \hspace{3em}%
  \mylabelbis{ax:F6}{P6}%
  $\tikzfig{tapes/cipriano/axF6left}
    \,\stackrel{\eqref{ax:F6}}{=}\,
    \tikzfig{tapes/cipriano/axF6right}$%
  \hspace{3em}%
  \mylabelbis{ax:F7}{P7}%
  $\tikzfig{tapes/cipriano/axF7left}
    \,\stackrel{\eqref{ax:F7}}{=}\,
    \tikzfig{tapes/cipriano/axF7right}$%
}

\end{tabular}
}
}
\caption{The monoidal theory of partial Boolean algebras.}
\label{tab:partialbooleanalgebra}
\end{figure}


We write $\ThPB$ for the monoidal theory consisting of the signature $PB$ and the axioms in Figures~\ref{tab:booleanalgebra} and~\ref{tab:partialbooleanalgebra};  $\eqPB$ for the generated congruence; $\Diag{\ThPB}$ for the quotient of $\Diag{PB}$ by $\eqPB$ and $Q_\ThPB\colon \Diag{ \SigPB} \to \Diag{\ThPB}$ the functor mapping each diagram into its $\eqPB$ equivalence class. Simple computations confirm that:

\begin{proposition}[Soundness]\label{prop:soundnesspartialb}
For all $c,d\in \Diag{PB}$, if $c\eqPB d$, then $\osemPB{c}=\osemPB{d}$.
\end{proposition}

The remainder of this section is devoted to proving the converse implication, namely completeness. 
Although this fact is not required for our proof, it is worth noting that the axiom \textsc{F8} in~\cite{piedeleu2025boolean}--corresponding to \eqref{ax:F8} in the following lemma--can be derived within $\ThPB$. 

\begin{lemma}\label{lemma:failureequalities}
  The following derived laws hold:
  \begin{center}
    \mylabelbis{ax:F9}{D6}%
    $\tikzfig{tapes/cipriano/axF9left}
      \stackrel{\eqref{ax:F9}}{\eqPB}
      \tikzfig{tapes/cipriano/axF9right}$
    \qquad
    \mylabelbis{ax:F8}{D7}%
    $\tikzfig{tapes/cipriano/axF8left}
      \stackrel{\eqref{ax:F8}}{\eqPB}
      \tikzfig{tapes/cipriano/axF8right}$
    \qquad
    \mylabelbis{ax:F10l}{D8l}%
    \mylabelbis{ax:F10r}{D8r}%
    $\tikzfig{tapes/cipriano/axF10left}
      \stackrel{\eqref{ax:F10l}}{\eqPB}
      \tikzfig{tapes/cipriano/axF10middle}
      \stackrel{\eqref{ax:F10r}}{\eqPB}
      \tikzfig{tapes/cipriano/axF10right}$
  \end{center}
\end{lemma}


The strategy for proving completeness is as follows. 
First, we show that any diagram $c$ in $\Diag{PB}$ can be decomposed into two diagrams $D_c$ and $T_c$ in $\Diag{\SigB}$ (Proposition~\ref{prop:decompositionpartialcircuits}). 
We then appeal to the completeness result for Boolean circuits (Theorem~\ref{thm:completenessbooleancircuits}).

Intuitively, $D_c$ and $T_c$ represent, respectively, the domain and the total component of $c$. 
The diagram $D_c$ returns $1$ if the input of $c$ lies in the domain of definition of $c$, and $0$ otherwise. 
The diagram $T_c$ returns the output of $c$ when the input lies in its domain, and a vector of $0$ otherwise.

\begin{definition}
For all $c\in \Diag{PB}[A^n,A^m]$, $D_c\in \Diag{\SigB}[A^n,A]$ and $T_c\in\Diag{\SigB}[A^n,A^m]$ are inductively defined as
\begin{equation}\label{eq:defTD}  \begin{array}{rcl@{\hspace{1.5cm}}rcl}
    D_c &\defeq& \CBdischargern\, \Flip{1} &       T_c &\defeq& c \qquad \text{for all generators $c\in \SigB$;}\\
    D_{\scalebox{0.6}{$\CBcocopier$}} &\defeq& \tikzfig{tapes/cipriano/xnorgatealone} &     T_{\scalebox{0.6}{$\CBcocopier$}} &\defeq& \Andgate\\
    D_{c;d} &\defeq &\quad \tikzfig{tapes/cipriano/Dfg} &  T_{c;d} &\defeq &\quad \tikzfig{tapes/cipriano/Tfg}\\
    D_{c\otimes d} &\defeq & \quad \tikzfig{tapes/cipriano/Dfperg} & T_{c\otimes d} &\defeq& \quad \tikzfig{tapes/cipriano/Tfperg}\\
  \end{array}
  \end{equation}
\end{definition}
Observe that the domain of $\CBcocopier$ is the $\mathrm{xnor}$ gate: it returns $1$ if and only if the two inputs are equal. 
Its total part is given by the $\wedge$ gate: it returns $1$ precisely when both inputs are $1$.
Similarly, the domain of $c \otimes d$ is given by the conjunction of the domains of $c$ and $d$. 
Its total part returns the total parts of $c$ and $d$ when the domain evaluates to $1$, and $0$ otherwise.

\begin{proposition}\label{prop:decompositionpartialcircuits}
  For all $c\in \Diag{BP}$, it holds that
  \begin{center}
  \tikzfig{tapes/cipriano/decompositionpartial}
  \end{center}
\end{proposition}
\marginpar{C: ho lasciato solo il caso composizione. il resto in app.}
\begin{proof}
  We proceed by induction on the structure of $c$. For the base case, if $c\in B$, then the statement follows by
  \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition1}
  \end{center} 
  If $c$ is $\CBcocopier$, then the statement is exactly axiom \eqref{ax:F6} in Figure~\ref{tab:partialbooleanalgebra}. Now, in the case $c;d$, then assuming that the statement holds for $c$ and $d$, we have
  \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition2}
    \end{center}
    \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition3}
    \end{center}
    \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition4}
    \end{center}
    \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition5}
    \end{center}
    where now the statement follows by inductive hypothesis. Finally, the case $c\otimes d$ is left in Appendix~\ref{app:sec:probboolcircuits}.
\end{proof}

%Hereafter, we write ${B}[1,A^n]$ for the set $n$-ary Boolean vectors, i.e., all those Boolean circuits in ${\Diag{PB}}[1,A^n]$ of the form $\bigotimes_{i=1}^n b_i$ for $b_i \in \{\Flip{0}, \Flip{1}\}$. \Diag{\SigB}
Before proceeding, recall that Theorem~\ref{thm:completenessbooleancircuits} implies that every $b\in \Diag{\SigB}[1,A^n]$ is $\eqB$-equal (hence $\eqPB$-equal) to a Boolean vector, i.e., a circuit of the form $\bigotimes_{i=1}^n b_i$ for $b_i \in \{\Flip{0}, \Flip{1}\}$ if $n>0$, and $\tikzfig{empty}$ if $n=0$. 

\begin{lemma}\label{lemma:complete1}
  Let $b\in \Diag{\SigB}[1,A^n]$ and $c\colon n\to m$ be a partial Boolean circuit. If $b;D_c \eqPB \Flip{0}$, then $b;T_c\eqPB\Flipm{0}$.
\end{lemma}








\begin{lemma}\label{lemma:complete3}
  For all $b\in \Diag{\SigB}[1,A^n]$ and $c,d\in \Diag{PB}[A^n,A^m]$, 
  \begin{center} if $\osemPB{b;c}=\osemPB{b;d}$, then $\osemPB{b;D_c}=\osemPB{b;D_d}$ and $\osemPB{b;T_c}=\osemPB{b;T_d}$.\end{center}
\end{lemma}




\begin{theorem}\label{thm:completenesspartialcircuits}[Completeness]
  For all $c,d\in \Diag{PB}[A^n,A^m]$, if $\osemPB{c}=\osemPB{d}$ then $c=_{\mathbb{\SigPB }}d$.
\end{theorem}
\begin{proof}
  For every $b\in \Diag{\SigB}[1,A^n]$, 
  \begin{align}
    \osemPB{b;c}&=\osemPB{b};\osemPB{c} \notag\\
    &=\osemPB{b};\osemPB{d} \tag{Hp.}\\
    &=\osemPB{b;d}. \notag
  \end{align}
  Lemma~\ref{lemma:complete3} implies that, for every $b\in \Diag{\SigB}[1,A^n]$, $\osemPB{b;D_c}=\osemPB{b;D_d}$ and $\osemPB{b;T_c}=\osemPB{b;T_d}$, hence $\osemPB{D_c} = \osemPB{D_d}$ and $\osemPB{T_c} = \osemPB{T_d}$. Now, since $D_c,D_d,T_c$ and $T_d$ are Boolean circuits in $\Diag{\SigB}$, then by Theorem~\ref{thm:completenessbooleancircuits} it holds that $D_c\eqB D_d$ and $T_c\eqB T_d$. Finally, by Proposition~\ref{prop:decompositionpartialcircuits}, since $c$ and $d$ decompose through the same domain and total part, we have that $c\eqPB d$.
\end{proof}
Moreover, one can characterise exactly the image of $\Diag{\SigPB}$ through $\osemPB{-}$. Let $\Cat{Par}_2$ be the full subcategory of $\Cat{Par}$ where objects are powers of the set $2$, i.e.,  $2^n$ for all $n \in \mathbb{N}$.


\begin{proposition}\label{prop:isopartialboolean}
The monoidal functor  $\osemPB{-}\colon \Diag{{\SigPB }} \to \Cat{Par}$ factors as
\[\xymatrix{ \Diag{\SigPB } \ar@{->>}[r]& \Diag{\mathbb{\SigPB }} \ar[r]^{\cong}& \Cat{Par}_2 \ar@{^{(}->}[r]& \Cat{Par} }\]
where the leftmost and rightmost functors are the obvious quotients and injections and the central arrow is a monoidal isomorphism.
\end{proposition}



Theorem \ref{thm:completenesspartialcircuits} also provides a useful characterisation of diagrams in $\Diag{\SigPB}[1,A^n]$. First consider the diagram $\ncopierbis\colon A \to A^n$ defined inductively as
\begin{center}
  \tikzfig{tapes/cipriano/ncopierbis}
\end{center}
then define the diagram $\Flipn{\bot}\colon 1 \to n$ as $\Flip{\bot};\ncopierbis$.
\begin{lemma}\label{lemma:caratterizzazionecircuiti0n}
  For all $c\in \Diag{\SigPB}[1,A^n]$, either $c\eqPB \Flipn{\bot}$ or $c\eqPB b$ for some $b\in \Diag{\SigB}[1,A^n]$.
\end{lemma}


\subsection{Probabilistic Boolean circuits}\label{ssec:probabilisticboolean}
Finally, we illustrate probabilistic Boolean circuits from \cite{piedeleu2025boolean}.
%
Consider the monoidal signature  \[ \SigPRB \defeq \SigPB \cup\{ \Flip{p} \mid p\in (0,1)\}\]  
 where $\Flip{p}$ denotes a probabilistic gate that receives no input and emits a Boolean signal on the right, which is $1$ with probability $p$ and $0$ with probability $1-p$. Thus, string diagrams in $\Diag{\SigPRB}$ represent arrows of $\KlD$, the Kleisli category of the subdistributions monad $\subdistr\colon \Sets \to \Sets$ (see e.g.,~\cite{hasuo2007generic}), which assigns to every set $X$ the set of \emph{subdistributions} over  $X$, i.e.\ the set of functions $d\colon X\to [0,1]$  such that $\sum_{x\in X}d(x)\leq 1$, and $d(x)\neq 0$ for only finitely many $x\in X$. 
 
 
 Recall that objects of $\KlD$ are sets; morphisms \(f \colon X \to Y\) are functions \(X \to \subdistr(Y)\). 
  We often write \(f(y \mid x)\) for \(f(x)(y)\), as this number represents the probability that \(f\) returns \(y\) given the input \(x\).
  Identities \(\id{X} \colon X \to \subdistr(X)\) map each element \(x \in X\) to \(\delta_{x}\).
  For two functions \(f \colon X \to \subdistr(Y)\) and \(g \colon Y \to \subdistr(Z)\), their composition in $\KlD$ is defined as \(f ; g (z \mid x) \defeq \sum_{y \in Y} f(y \mid x) \cdot g(z \mid y)\).


To formally define their semantics, consider the symmetric monoidal structure $(\KlD, \otimes, \uno)$, where $\otimes$ is the cartesian product of sets with unit the singleton $\uno \defeq \{\bullet\}$ and, for arrows  \(f \colon X \to Y\) and \(g \colon X' \to Y'\), $f\per g\colon X\otimes X' \to Y \otimes Y'$ is defined, for all $x\in X$, $x'\in X'$, $y\in Y$, $y'\in Y'$, as follows.
\begin{equation}\label{ex:products}
\begin{aligned}
f \per g(y,y' \mid x,x') &\defeq f(y \mid x) \cdot g(y' \mid x')
\end{aligned}
\end{equation}
And observe that there is an obvious monoidal embedding $\ParJ\colon \Cat{Par} \to \KlD$ which is the identity on objects and associates to a partial function $f\colon X \to Y$ the function $\ParJ(f)\colon X \to \Dis(Y)$, mapping $x$ to $\delta_{f(x)}$, if $f(x)$ is defined and to the null distribution $\star$ otherwise. 




The semantics of $\SigPRB$ is given by the monoidal functor $\osem{-}\colon \Diag{\SigPRB} \to \KlD$ defined on objects as $A^n \mapsto 2^n$. On arrows, it is defined by first interpreting generators  $c\in \SigPB$ as $\ParJ(\osemPB{c})$, i.e.
\[
    \begin{array}{rclrclrcl}
      \osem{\Andgate}\colon 2 \times 2& \to & 2  & \osem{\Notgate}\colon  2& \to & 2 & \osem{\Flip{1}} \colon 1 & \to & 2 \\
      (x,y)&\mapsto&\delta_{x\wedge y} &  x & \mapsto & \delta_{\neg x} & \bullet &\mapsto&\delta_{1}\\[4pt]
       \osem{\CBcopier} \colon 2  & \to & 2\times 2 & \osem{\CBdischarger} \colon 2 & \to & 1 & \osem{\CBcocopier} \colon 2 \times 2 & \to & 2  \\
      x &\mapsto&\delta_{(x,x)} & x &\mapsto&\delta_{\bullet} & (x,y) &\mapsto& \begin{cases}\delta_{x} &\text{if }x=y\\ \star & \text{else}\end{cases}, 
    \end{array}
  \]

 the generator $\Flip{p}$ as 
\begin{equation}\label{eq:semanticsFlip}
\begin{array}{rcl}
      \osem{\Flip{p}}\colon 1& \to & 2   \\
      \bullet&\mapsto& \delta_1 +_p \delta_0  \end{array}
    \end{equation}
and then inductively on the structure of the monoidal category $(\KlD, \otimes, \uno)$. Simple computations confirm that $\osem{-}$ extends both $\osemB{-}$ and $\osemPB{-}$, in the sense that the following diagrams commute.
\[
\xymatrix{\Diag{\SigB} \ar@{^{(}->}[r] \ar[d]_{\osemB{-}}& \Diag{\SigPB} \ar@{^{(}->}[r] \ar[d]|{\osemPB{-}} & \Diag{\SigPRB} \ar[d]^{\osem{-}}\\
\Sets \ar@{^{(}->}[r]_{\Pa}& \Cat{Par} \ar@{^{(}->}[r]_{\ParJ}& \KlD
}
\]








\medskip
Figures~4 and~5 in \cite{piedeleu2025boolean} provide a sound and complete equational axiomatisation of probabilistic Boolean circuits. The system essentially consists of the axioms of Boolean algebras (reported in Figure~\ref{tab:booleanalgebra}), together with four non-trivial axioms governing the behaviour of $\Flip{p}$ and additional axioms for $\CBcocopier$, which differ from those presented in Figure~\ref{tab:partialbooleanalgebra}.

Importantly, the equivalence induced by these axioms is strictly coarser than the one given by $\osem{-}$. In fact, two diagrams $c$ and $d$ are equivalent under the axioms of \cite{piedeleu2025boolean} if and only if $\osem{c} \propto \osem{d}$. The relation $\propto$ is defined on arrows of $\KlD$ by setting $f \propto g$ whenever there exists a real number $\lambda > 0$ such that $f(y\mid x) = \lambda \cdot g(y\mid x)$ for all $x \in X$ and $y \in Y$. %In the next section, we provide a complete  axiomatisation for the equivalence induced by $\osem{-}$ by means of probabilistic tape diagrams.





==> sections/probabilisticbooleancircuits.tex <==

\section{Probabilistic Boolean Circuits}\label{sec:probboolcircuits}

In this section we recall the definition of probabilistic Boolean circuits from \cite{piedeleu2025boolean}. To do that, we first deal with Boolean circuits in Section~\ref{ssec:boolean}, then we introduce  partial Boolean circuits in Section~\ref{ssec:partialboolean} and provide a complete axiomatisation. Finally, in Section~\ref{ssec:probabilisticboolean} we introduce probabilistic Boolean circuits  and their semantics.


\marginpar{C:richiamare questo per fissare le noazioni Diag}

Before proceeding, recall that a monoidal signature is a tuple $(\sort, \sign, \ari, \coar)$ where $\sort$ is a set of basic sorts, hereafter denoted by $A,B,\dots$, $\sign$ is a set of generators, denoted by $s,t, \dots$, and $\ari,\coar \colon \sign \to \sort^*$ assign to each symbol its arity and coarity (words over $\sort$). Consider the strict symmetric monoidal category $\DiagS$:  objects are words in $\sort^*$; arrows are \emph{string diagrams} \cite{joyal1991geometry,selinger2010survey}. These can be regarded  as the terms generated by the following grammar (where $A,B \in \sort$ and $s \in \Sigma$)
\begin{equation}\label{stringdiagramGrammar}
\setlength{\arraycolsep}{3pt} % spaziatura orizzontale
\renewcommand{\arraystretch}{1.1} % opzionale: un po' di respiro verticale
\begin{array}{rcccccccccccccccc}
c & ::= & \id{A} & \mid & \id{\uno} & \mid & \gen & \mid & \symmt{A}{B} & \mid & c ; c & \mid & c \per c
\end{array}
\end{equation}
modulo the axioms of strict symmetric monoidal categories. A \emph{monoidal theory} $\mathbb{T}=(\sign, E)$ consists of a monoidal signature equipped with a set $E$ of pairs of arrows of $\DiagS$ with same source and target. Let $=_{\mathbb{T}}$ be an equivalence relation on arrows  of $\DiagS$ obtained as the congruence closure (w.r.t. $;$ and $\otimes$) of $E$. We write $\DiagT$ for the category obtained as the quotient of $\DiagS$ by $=_{\mathbb{T}}$.


\subsection{Boolean Circuits}\label{ssec:boolean}
Consider the monoidal signature with a single sort, $\sort = \{ A\}$, and  generators 
\[ \SigB \defeq \{\Andgate  , \Notgate , \Flip{1},   \CBcopier, \CBdischarger \} \text{.}\]  
Arities and coarities are determined by the number of ports on the left and on the right: for instance, $\Andgate$ has arity $A^2=AA$ and coarity $A$, while $\CBdischarger $ has arity $A$ and coarity $A^0 =1$. 

The arrows of $\Diag{\SigB}$ are interpreted as Boolean functions. 
The first three generators of $\SigB$ correspond to the operations and constants of Boolean algebras, namely $\wedge$, $\neg$, and $1$. 
The generator \emph{copy}, denoted by $\CBcopier$, takes a Boolean signal as input and produces two identical outputs. 
The generator \emph{discard}, denoted by $\CBdischarger$, takes a Boolean signal as input and discards it.


Formally, the semantics of these diagrams is given by the monoidal functor  $\osemB{-}\colon \Diag{{\SigB}} \to \Sets$ defined on objects as $A^n \mapsto 2^n$ where $2$ is the set of Booleans  $\{0,1\}$; for arrows it is defined by first interpreting the generators as functions in $\Sets$
  \[
    \begin{array}{rclrclrcl}
      \osemB{\Andgate}\colon 2 \times 2& \to & 2  & \osemB{\Notgate}\colon  2& \to & 2 & \osemB{\Flip{1}} \colon 1 & \to & 2 \\
      (x,y)&\mapsto& x\wedge y &  x & \mapsto & \neg x & \bullet &\mapsto&1\\[4pt]
       \osemB{\CBcopier} \colon 2  & \to & 2\times 2 & \osemB{\CBdischarger} \colon 2 & \to & 1 & %\osemB{\Flip{p}} \colon 1 & \to & 2  
       \\
      x &\mapsto&(x,x) & x &\mapsto&{\bullet} & %\bullet &\mapsto& \delta_1 +_p \delta_0
    \end{array}
  \]
and then inductively by means of the structure of the monoidal category $(\Sets, \otimes ,\uno)$: for instance, $\osemB{c_1\otimes c_2}=\osemB{c_1}\otimes \osemB{c_2}$ where the second $\otimes$ is the standard cartesian product of functions. 

The monoidal theory $\ThB$ consists of the signature $\SigB$ together with the axioms listed in Figure~\ref{tab:booleanalgebra}. 
The equalities in the first block are the standard axioms of Boolean algebras. 
The constant $\Flip{0}$ and the $\Orgate$ gate are defined as expected (see Figure~\ref{table:multiplexer}). 
Note that, in the string-diagrammatic setting, the structural maps $\CBcopier$ and $\CBdischarger$ must be made explicit.
The equalities in the second block state that $\CBcopier$ and $\CBdischarger$ form a commutative comonoid. 
The equalities in the third and fourth blocks impose naturality of $\CBcopier$ and $\CBdischarger$, respectively.


The congruence with respect to $;$ and $\otimes$ generated by the axioms in Figure~\ref{tab:booleanalgebra} is denoted by $\eqB$. 
We write $\Diag{\ThB}$ for the quotient of $\Diag{\SigB}$ by $\eqB$.

As expected, the equalities in Figure~\ref{tab:booleanalgebra} provide a sound and complete axiomatization of the equality induced by $\osemB{-}$. See e.g. \cite[Theorem 3.2]{piedeleu2025boolean}.

\begin{theorem}\label{thm:completenessbooleancircuits}
For all  $c,d\in \Diag{\SigB}$, $\osemB{c}=\osemB{d}$ iff $c\eqB d$.
\end{theorem}


\begin{figure}
  \scalebox{0.8}{%
  \begin{tabular}{ccccc}

  % =====================
  % ---- B axioms ----
  % =====================

  \mylabelbis{ax:B1}{B1}%
  $\tikzfig{tapes/cipriano/axB1left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B1}}{=}$\,}\tikzfig{tapes/cipriano/axB1right}$
  & &
  \mylabelbis{ax:B2l}{B2l}\mylabelbis{ax:B2r}{B2r}%
  $\tikzfig{tapes/cipriano/axB2left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B2l}}{=}$\,}\tikzfig{tapes/cipriano/axB2middle}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B2r}}{=}$\,}\tikzfig{tapes/cipriano/axB2right}$
  & &
  \mylabelbis{ax:B3}{B3}%
  $\tikzfig{tapes/cipriano/axB3left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B3}}{=}$\,}\tikzfig{tapes/cipriano/axB3right}$
  \\

  \mylabelbis{ax:B4}{B4}%
  $\tikzfig{tapes/cipriano/axB4left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B4}}{=}$\,}\tikzfig{tapes/cipriano/axB4right}$
  & &
  \mylabelbis{ax:B5}{B5}%
  $\tikzfig{tapes/cipriano/axB5left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B5}}{=}$\,}\tikzfig{tapes/cipriano/axB5right}$
  & &
  \mylabelbis{ax:B6}{B6}%
  $\tikzfig{tapes/cipriano/axB6left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B6}}{=}$\,}\tikzfig{tapes/cipriano/axB6right}$
  \\

  & &
  \mylabelbis{ax:B7}{B7}%
  $\tikzfig{tapes/cipriano/axB7left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:B7}}{=}$\,}\tikzfig{tapes/cipriano/axB7right}$
  & &
  \\

  \midrule

  % =====================
  % ---- A axioms ----
  % =====================

  \mylabelbis{ax:A1}{B8}%
  $\tikzfig{tapes/cipriano/axA1left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A1}}{=}$\,}\tikzfig{tapes/cipriano/axA1right}$
  & &
  \mylabelbis{ax:A2l}{B9l}\mylabelbis{ax:A2r}{B9r}%
  $\tikzfig{tapes/cipriano/axA2left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A2l}}{=}$\,}\tikzfig{tapes/cipriano/axA2middle}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A2r}}{=}$\,}\tikzfig{tapes/cipriano/axA2right}$
  & &
  \mylabelbis{ax:A3}{B10}%
  $\tikzfig{tapes/cipriano/axA3left}\raisebox{-1.5ex}{\,$\stackrel{\eqref{ax:A3}}{=}$\,}\tikzfig{tapes/cipriano/axA3right}$
  \\

  \midrule

  % =====================
  % ---- C axioms ----
  % =====================

  \mylabelbis{ax:C1}{B11}%
  $\tikzfig{tapes/cipriano/axC1left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:C1}}{=}$\,}\tikzfig{tapes/cipriano/axC1right}$
  & &
  \mylabelbis{ax:C2}{B12}%
  $\tikzfig{tapes/cipriano/axC2left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:C2}}{=}$\,}\tikzfig{tapes/cipriano/axC2right}$
  & &
  \mylabelbis{ax:C3}{B13}%
  $\tikzfig{tapes/cipriano/axC3left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:C3}}{=}$\,}\tikzfig{tapes/cipriano/axC3right}$
  \\

  \midrule

  % =====================
  % ---- D axioms ----
  % =====================

  \mylabelbis{ax:D1}{B14}%
  $\tikzfig{tapes/cipriano/axD1left}\raisebox{-0.6ex}{\,$\stackrel{\eqref{ax:D1}}{=}$\,}\tikzfig{tapes/cipriano/axD1right}$
  & &
  \mylabelbis{ax:D2}{B15}%
  $\tikzfig{tapes/cipriano/axD2left}\raisebox{-0.6ex}{$\stackrel{\eqref{ax:D2}}{=}$}\tikzfig{tapes/cipriano/axD2right}$
  & &
  \mylabelbis{ax:D3}{B16}%
  $\tikzfig{tapes/cipriano/axD3left}\raisebox{-0.6ex}{$\stackrel{\eqref{ax:D3}}{=}$}
  \raisebox{-0.5em}{\tikzfig{empty}}$
  \\

  \end{tabular}}%
  \caption{The monoidal theory of Boolean algebras.}
  \label{tab:booleanalgebra}
\end{figure}
Moreover, one can characterise exactly the image of $\Diag{\SigB}$ through $\osemB{-}$. Let $\Sets_2$ be the full subcategory of sets where objects are powers of the set $2$, i.e.,  $2^n$ for all $n \in \mathbb{N}$.


\begin{proposition}\label{prop:foolboolean}
The monoidal functor  $\osemB{-}\colon \Diag{{\SigB}} \to \Sets$ factors as
\[\xymatrix{ \Diag{\SigB} \ar@{->>}[r]& \Diag{\ThB} \ar[r]^{\cong}& \Sets_2 \ar@{^{(}->}[r]& \Sets }\]
where the leftmost and rightmost functor are the obvious quotients and injections and the central arrows is a monoidal isomorphism.
\end{proposition}
\begin{proof}
Faithfulness of the central functor is a direct consequence of Theorem~\ref{thm:completenessbooleancircuits}. Fullness follows from the fact that every function $f\colon 2^n \to 2^m$ corresponds to a vector of $m$ Boolean formulas in $n$ variables, which can be easily encoded as a string diagram in $\Diag{\ThB}$ using Boolean operators, $\CBcopier$ and $\CBdischarger$.
\end{proof}



We conclude this section by fixing some syntactic sugar, collected in Figure~\ref{table:multiplexer}. 
The \emph{xnor} gate $\xnor$  takes two Boolean inputs and outputs $1$ if they are equal and $0$ otherwise. 
The \emph{multiplexer} $\tikzfig{tapes/cipriano/multi}$ takes three inputs and returns one output: if the first input is $1$, then it outputs the second input, otherwise the third input. 
The $m$-ary multiplexer $\Ifgatem$ works similarly, but it takes $2m+1$ inputs: if the first input is $1$, then it outputs the first $m$ inputs, otherwise it outputs the second $m$ inputs. 
Figure~\ref{table:multiplexer} also defines $m$-ary discard $\CBdischargerm$ and copier $\mcopier$. Note that, for the sake of readability of string diagrams, we label wires by  some natural number $n$ as an abbreviation for $A^n$.

\begin{lemma}\label{lemma:multiplexer}
 Let $c$ be a diagram in $\Diag{\SigB}[n,m]$. The following derived laws hold:

\mylabelbis{ax:M1}{D1}
\mylabelbis{ax:M2}{D2}
\mylabelbis{ax:M3}{D3}
\mylabelbis{ax:N1}{D4}
\mylabelbis{ax:N2}{D5}

\[
\begin{array}{c@{\qquad}c@{\qquad}c}

\raisebox{-0.3em}{\tikzfig{tapes/cipriano/D1left}} 
\stackrel{\eqref{ax:M1}}{\eqB}
\tikzfig{tapes/cipriano/D1right}

&
\raisebox{-0.3em}{\tikzfig{tapes/cipriano/D2left}}
\stackrel{\eqref{ax:M2}}{\eqB}
\tikzfig{tapes/cipriano/D2right}

&
\raisebox{-0.3em}{\tikzfig{tapes/cipriano/D3left}}
\stackrel{\eqref{ax:M3}}{\eqB}
\tikzfig{tapes/cipriano/D3right}

\\[1em]

\tikzfig{tapes/cipriano/D4left}
\stackrel{\eqref{ax:N1}}{\eqB}
\tikzfig{tapes/cipriano/D4right}

&
\tikzfig{tapes/cipriano/D5left}
\stackrel{\eqref{ax:N2}}{\eqB}
\tikzfig{tapes/cipriano/D5right}

&

\end{array}
\]
\end{lemma}




\begin{figure}[t]
\centering
\resizebox{0.96\linewidth}{!}{%
\begin{tabular}{@{}l@{}}

% ---- Row 1 ----
$\Orgate \defeq (\Notgate \otimes \Notgate); \Andgate; \Notgate 
\qquad 
\Flip{0} \defeq \Flip{1}; \Notgate
\qquad
\tikzfig{tapes/cipriano/multi} 
\defeq 
\tikzfig{tapes/cipriano/multiexpl}$ \\[4pt]

% ---- Row 2 ----
$\tikzfig{tapes/cipriano/xnorgate}
\qquad
\raisebox{-1em}{\tikzfig{tapes/cipriano/ncopierzero}} 
\raisebox{-0.5em}{$\defeq$}
\raisebox{-0.5em}{\tikzfig{empty}}
\qquad 
\raisebox{-1em}{\tikzfig{tapes/cipriano/ncopier}}$ \\[6pt]

% ---- Row 3 ----
$\raisebox{-1.2em}{\tikzfig{tapes/cipriano/mmultiplexerleftzero}} 
\defeq 
\tikzfig{tapes/cipriano/mmultiplexerrightzero}
\qquad 
\raisebox{-1.2em}{\tikzfig{tapes/cipriano/mmultiplexerleft}} 
\defeq 
\tikzfig{tapes/cipriano/mmultiplexerright}$ \\[6pt]

% ---- Row 4 ----
$\mFlip{1}{0} \defeq \tikzfig{empty}
\qquad
\mFlip{1}{m+1} \defeq \Flip{1} \otimes \mFlip{1}{m}
\qquad
\mCBdischarger{0} \defeq \tikzfig{empty}
\qquad
\mCBdischarger{m+1} \defeq \CBdischarger\otimes \mCBdischarger{m}$

\end{tabular}
}
\caption{Definitions of OR gate, $\Flip{0}$ and multiplexer (top); definitions of XNOR gate and inductive definition of $n$-ary copier (middle); inductive definitions of $m$-ary multiplexer (third row); definitions of $\Flipzero{1}$, $\Flipm{1}$ and $n$-ary dischargers (bottom).}
\label{table:multiplexer}
\end{figure}

%
%
% SUBSECTION
%
%
\subsection{Partial Boolean Circuits}\label{ssec:partialboolean}
Now consider the monoidal signature obtained by adding to $\SigB$ the generator \emph{cocopy} $\CBcocopier$ of arity $A^2$ and coarity $A$. 
\[ PB\defeq \SigB \cup\{\CBcocopier\}\text{}\] 
Intuitively, $\CBcocopier$ is the dual of $\CBcopier$: it compares two inputs and, if these are equal, it outputs that value; otherwise, it produces no output. Thus, string diagrams in $\Diag{PB}$ represent \emph{partial} Boolean functions. 

To formally define their semantics, let us first fix $(\Cat{Par}, \otimes, 1)$ to be the symmetric monoidal category of sets and partial functions, where the monoidal product $\otimes$ is the cartesian product of sets and, for all partial functions $f_1\colon X_1 \to Y_1$ and $f_2\colon X_2 \to Y_2$, $f_1\otimes f_2 \colon X_1 \times X_2 \to Y_1 \times Y_2$ is defined as
\begin{equation}\label{eq:productpar}
f_1\otimes f_2 (x_1,x_2) \defeq \begin{cases} (\,f_1(x_1), \, f_2(x_2)\,) & \text{ if }f_1(x_1)\neq \bot\text{, } f_2(x_2)\neq \bot \\
 \bot & \text{ otherwise}\end{cases}
\end{equation}
for all $(x_1,x_2)\in X_1\times X_2$. Above, and in the rest of the paper, we write $f(x)=\bot$ to say that a partial function $f\colon X \to Y$ is undefined for some $x\in X$. 
One can readily check that the obvious injection $\Pa\colon \Sets \to \Cat{Par}$ is a symmetric monoidal functor.


Now, the semantics of diagrams in $\Diag{PB}$ is given by the monoidal functor $\osemPB{-}\colon \Diag{PB} \to \Cat{Par}$ defined on objects as $A^n \mapsto 2^n$, like $\osemB{-}$; 
for arrows it is defined by first interpreting generators $c \in \SigB$ as $\osemPB{c}\defeq \Pa(\osemB{c})$, the generator $\CBcocopier $ as
  \begin{equation}\label{eq:semcocopier}
    \begin{array}{rcl}
      \osemPB{\CBcocopier}\colon 2 \times 2& \to & 2   \\
      (x,y)&\mapsto& \begin{cases} x &\text{if } x=y\\ \bot & \text{else}\end{cases}    \end{array}
  \end{equation}
and then inductively by means of the structure of the monoidal category $(\Cat{Par}, \otimes ,\uno)$: for instance $\osemB{c_1\otimes c_2}=\osemB{c_1}\otimes \osemB{c_2}$ where the second $\otimes$ is the one in \eqref{eq:productpar}. %A simple inductive argument confirms that $\osemPB{-}$ is an extension of $\osemB{-}$, i.e., the following diagram commutes
%\[
%\xymatrix{\Diag{PB} \ar[r]^{\osemPB{-}} & \Cat{Par}\\ 
%\Diag{B} \ar[r]_{\osemB{-}} \ar@{>->}[u] & \Sets \ar@{>->}[u]_P
%}
%\]
For example, the semantics of the following diagrams
\begin{equation}\label{def:bottom}
  \raisebox{0cm}{\tikzfig{tapes/cipriano/defcoflip}}
\end{equation}
is illustrated below.
  \[
    \begin{array}{rclrclrcl}
      \osemPB{\coflip{1} }\colon 2 & \to & 1  & \osemPB{\coflip{0} }\colon 2 & \to & 1 & \osemPB{\Flip{\bot}}\colon 1 & \to & 2 \\
      x&\mapsto& \begin{cases} \bullet &\text{if } x=1\\ \bot & \text{else}\end{cases}    
      &
      x&\mapsto& \begin{cases} \bullet &\text{if } x=0\\ \bot & \text{else}\end{cases}    
      &
      \bullet &\mapsto & \bot     
      \end{array}
  \]






In this section, we present a complete axiomatization of the equality induced by $\osemPB{-}$, which, to the best of our knowledge, has not been previously established.
The axioms are illustrated in Figure~\ref{tab:partialbooleanalgebra}: the equalities in the first row assert that $\CBcocopier$ is associative, commutative and idempotent; in the second row, there are the usual Frobenius equalities ruling the interaction of $\CBcocopier$ with $\CBcopier$; the two axioms in the third row are more peculiar: the rightmost states that $x\wedge y = 1$ iff $x=y=1$; the leftmost provides a decomposition of  $\CBcocopier$ in terms of $\Andgate$, $\coflip{1}$ and the xnor gate \tikzfig{tapes/cipriano/xnorgatealone}.



%%%%%%%NUOVA TABELLA CON TAG%%%%%%%%%%
\begin{figure}
\centering
\scalebox{0.8}{
{
\setlength{\tabcolsep}{12pt}      % spazio orizzontale
\setlength{\extrarowheight}{9pt}  % spazio verticale aggiuntivo
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{ccc}

% Prima riga
\hspace{1.5em}%
\mylabelbis{ax:F1}{P1}%
$\tikzfig{tapes/cipriano/axF1left}
 \raisebox{-0.6em}{\,\,$\stackrel{\eqref{ax:F1}}{=}$\,\,}
 \tikzfig{tapes/cipriano/axF1right}$
&
\hspace{1.5em}%
\mylabelbis{ax:F2}{P2}%
$\tikzfig{tapes/cipriano/axF2left}
 \raisebox{-0.6em}{\,$\stackrel{\eqref{ax:F2}}{=}$\,}
 \tikzfig{tapes/cipriano/axF2right}$
&
\hspace{1.5em}%
\mylabelbis{ax:F3}{P3}%
$\tikzfig{tapes/cipriano/axF3left}
 \raisebox{-0.6em}{\,\,$\stackrel{\eqref{ax:F3}}{=}$\,\,}
 \tikzfig{tapes/cipriano/axF3right}$
\\[1.2em]

% Seconda riga
\multicolumn{3}{c}{%
  \scalebox{0.85}{%
    \mylabelbis{ax:F4}{P4}%
    \mylabelbis{ax:F5}{P5}%
    $\tikzfig{tapes/cipriano/axF4left}
      \,\stackrel{\eqref{ax:F4}}{=}\,
      \tikzfig{tapes/cipriano/axF4right}
      \,\stackrel{\eqref{ax:F5}}{=}\,
      \tikzfig{tapes/cipriano/axF5}$%
  }%
  \hspace{3em}%
  \mylabelbis{ax:F6}{P6}%
  $\tikzfig{tapes/cipriano/axF6left}
    \,\stackrel{\eqref{ax:F6}}{=}\,
    \tikzfig{tapes/cipriano/axF6right}$%
  \hspace{3em}%
  \mylabelbis{ax:F7}{P7}%
  $\tikzfig{tapes/cipriano/axF7left}
    \,\stackrel{\eqref{ax:F7}}{=}\,
    \tikzfig{tapes/cipriano/axF7right}$%
}

\end{tabular}
}
}
\caption{The monoidal theory of partial Boolean algebras.}
\label{tab:partialbooleanalgebra}
\end{figure}


We write $\ThPB$ for the monoidal theory consisting of the signature $PB$ and the axioms in Figures~\ref{tab:booleanalgebra} and~\ref{tab:partialbooleanalgebra};  $\eqPB$ for the generated congruence; $\Diag{\ThPB}$ for the quotient of $\Diag{PB}$ by $\eqPB$ and $Q_\ThPB\colon \Diag{ \SigPB} \to \Diag{\ThPB}$ the functor mapping each diagram into its $\eqPB$ equivalence class. Simple computations confirm that:

\begin{proposition}[Soundness]\label{prop:soundnesspartialb}
For all $c,d\in \Diag{PB}$, if $c\eqPB d$, then $\osemPB{c}=\osemPB{d}$.
\end{proposition}

The remainder of this section is devoted to proving the converse implication, namely completeness. 
Although this fact is not required for our proof, it is worth noting that the axiom \textsc{F8} in~\cite{piedeleu2025boolean}--corresponding to \eqref{ax:F8} in the following lemma--can be derived within $\ThPB$. 

\begin{lemma}\label{lemma:failureequalities}
  The following derived laws hold:
  \begin{center}
    \mylabelbis{ax:F9}{D6}%
    $\tikzfig{tapes/cipriano/axF9left}
      \stackrel{\eqref{ax:F9}}{\eqPB}
      \tikzfig{tapes/cipriano/axF9right}$
    \qquad
    \mylabelbis{ax:F8}{D7}%
    $\tikzfig{tapes/cipriano/axF8left}
      \stackrel{\eqref{ax:F8}}{\eqPB}
      \tikzfig{tapes/cipriano/axF8right}$
    \qquad
    \mylabelbis{ax:F10l}{D8l}%
    \mylabelbis{ax:F10r}{D8r}%
    $\tikzfig{tapes/cipriano/axF10left}
      \stackrel{\eqref{ax:F10l}}{\eqPB}
      \tikzfig{tapes/cipriano/axF10middle}
      \stackrel{\eqref{ax:F10r}}{\eqPB}
      \tikzfig{tapes/cipriano/axF10right}$
  \end{center}
\end{lemma}


The strategy for proving completeness is as follows. 
First, we show that any diagram $c$ in $\Diag{PB}$ can be decomposed into two diagrams $D_c$ and $T_c$ in $\Diag{\SigB}$ (Proposition~\ref{prop:decompositionpartialcircuits}). 
We then appeal to the completeness result for Boolean circuits (Theorem~\ref{thm:completenessbooleancircuits}).

Intuitively, $D_c$ and $T_c$ represent, respectively, the domain and the total component of $c$. 
The diagram $D_c$ returns $1$ if the input of $c$ lies in the domain of definition of $c$, and $0$ otherwise. 
The diagram $T_c$ returns the output of $c$ when the input lies in its domain, and a vector of $0$ otherwise.

\begin{definition}
For all $c\in \Diag{PB}[A^n,A^m]$, $D_c\in \Diag{\SigB}[A^n,A]$ and $T_c\in\Diag{\SigB}[A^n,A^m]$ are inductively defined as
\begin{equation}\label{eq:defTD}  \begin{array}{rcl@{\hspace{1.5cm}}rcl}
    D_c &\defeq& \CBdischargern\, \Flip{1} &       T_c &\defeq& c \qquad \text{for all generators $c\in \SigB$;}\\
    D_{\scalebox{0.6}{$\CBcocopier$}} &\defeq& \tikzfig{tapes/cipriano/xnorgatealone} &     T_{\scalebox{0.6}{$\CBcocopier$}} &\defeq& \Andgate\\
    D_{c;d} &\defeq &\quad \tikzfig{tapes/cipriano/Dfg} &  T_{c;d} &\defeq &\quad \tikzfig{tapes/cipriano/Tfg}\\
    D_{c\otimes d} &\defeq & \quad \tikzfig{tapes/cipriano/Dfperg} & T_{c\otimes d} &\defeq& \quad \tikzfig{tapes/cipriano/Tfperg}\\
  \end{array}
  \end{equation}
\end{definition}
Observe that the domain of $\CBcocopier$ is the $\mathrm{xnor}$ gate: it returns $1$ if and only if the two inputs are equal. 
Its total part is given by the $\wedge$ gate: it returns $1$ precisely when both inputs are $1$.
Similarly, the domain of $c \otimes d$ is given by the conjunction of the domains of $c$ and $d$. 
Its total part returns the total parts of $c$ and $d$ when the domain evaluates to $1$, and $0$ otherwise.

\begin{proposition}\label{prop:decompositionpartialcircuits}
  For all $c\in \Diag{BP}$, it holds that
  \begin{center}
  \tikzfig{tapes/cipriano/decompositionpartial}
  \end{center}
\end{proposition}
\marginpar{C: ho lasciato solo il caso composizione. il resto in app.}
\begin{proof}
  We proceed by induction on the structure of $c$. For the base case, if $c\in B$, then the statement follows by
  \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition1}
  \end{center} 
  If $c$ is $\CBcocopier$, then the statement is exactly axiom \eqref{ax:F6} in Figure~\ref{tab:partialbooleanalgebra}. Now, in the case $c;d$, then assuming that the statement holds for $c$ and $d$, we have
  \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition2}
    \end{center}
    \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition3}
    \end{center}
    \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition4}
    \end{center}
    \begin{center}
    \tikzfig{tapes/cipriano/propdecomposition5}
    \end{center}
    where now the statement follows by inductive hypothesis. Finally, the case $c\otimes d$ is left in Appendix~\ref{app:sec:probboolcircuits}.
\end{proof}

%Hereafter, we write ${B}[1,A^n]$ for the set $n$-ary Boolean vectors, i.e., all those Boolean circuits in ${\Diag{PB}}[1,A^n]$ of the form $\bigotimes_{i=1}^n b_i$ for $b_i \in \{\Flip{0}, \Flip{1}\}$. \Diag{\SigB}
Before proceeding, recall that Theorem~\ref{thm:completenessbooleancircuits} implies that every $b\in \Diag{\SigB}[1,A^n]$ is $\eqB$-equal (hence $\eqPB$-equal) to a Boolean vector, i.e., a circuit of the form $\bigotimes_{i=1}^n b_i$ for $b_i \in \{\Flip{0}, \Flip{1}\}$ if $n>0$, and $\tikzfig{empty}$ if $n=0$. 

\begin{lemma}\label{lemma:complete1}
  Let $b\in \Diag{\SigB}[1,A^n]$ and $c\colon n\to m$ be a partial Boolean circuit. If $b;D_c \eqPB \Flip{0}$, then $b;T_c\eqPB\Flipm{0}$.
\end{lemma}








\begin{lemma}\label{lemma:complete3}
  For all $b\in \Diag{\SigB}[1,A^n]$ and $c,d\in \Diag{PB}[A^n,A^m]$, 
  \begin{center} if $\osemPB{b;c}=\osemPB{b;d}$, then $\osemPB{b;D_c}=\osemPB{b;D_d}$ and $\osemPB{b;T_c}=\osemPB{b;T_d}$.\end{center}
\end{lemma}




\begin{theorem}\label{thm:completenesspartialcircuits}[Completeness]
  For all $c,d\in \Diag{PB}[A^n,A^m]$, if $\osemPB{c}=\osemPB{d}$ then $c=_{\mathbb{\SigPB }}d$.
\end{theorem}
\begin{proof}
  For every $b\in \Diag{\SigB}[1,A^n]$, 
  \begin{align}
    \osemPB{b;c}&=\osemPB{b};\osemPB{c} \notag\\
    &=\osemPB{b};\osemPB{d} \tag{Hp.}\\
    &=\osemPB{b;d}. \notag
  \end{align}
  Lemma~\ref{lemma:complete3} implies that, for every $b\in \Diag{\SigB}[1,A^n]$, $\osemPB{b;D_c}=\osemPB{b;D_d}$ and $\osemPB{b;T_c}=\osemPB{b;T_d}$, hence $\osemPB{D_c} = \osemPB{D_d}$ and $\osemPB{T_c} = \osemPB{T_d}$. Now, since $D_c,D_d,T_c$ and $T_d$ are Boolean circuits in $\Diag{\SigB}$, then by Theorem~\ref{thm:completenessbooleancircuits} it holds that $D_c\eqB D_d$ and $T_c\eqB T_d$. Finally, by Proposition~\ref{prop:decompositionpartialcircuits}, since $c$ and $d$ decompose through the same domain and total part, we have that $c\eqPB d$.
\end{proof}
Moreover, one can characterise exactly the image of $\Diag{\SigPB}$ through $\osemPB{-}$. Let $\Cat{Par}_2$ be the full subcategory of $\Cat{Par}$ where objects are powers of the set $2$, i.e.,  $2^n$ for all $n \in \mathbb{N}$.


\begin{proposition}\label{prop:isopartialboolean}
The monoidal functor  $\osemPB{-}\colon \Diag{{\SigPB }} \to \Cat{Par}$ factors as
\[\xymatrix{ \Diag{\SigPB } \ar@{->>}[r]& \Diag{\mathbb{\SigPB }} \ar[r]^{\cong}& \Cat{Par}_2 \ar@{^{(}->}[r]& \Cat{Par} }\]
where the leftmost and rightmost functors are the obvious quotients and injections and the central arrow is a monoidal isomorphism.
\end{proposition}



Theorem \ref{thm:completenesspartialcircuits} also provides a useful characterisation of diagrams in $\Diag{\SigPB}[1,A^n]$. First consider the diagram $\ncopierbis\colon A \to A^n$ defined inductively as
\begin{center}
  \tikzfig{tapes/cipriano/ncopierbis}
\end{center}
then define the diagram $\Flipn{\bot}\colon 1 \to n$ as $\Flip{\bot};\ncopierbis$.
\begin{lemma}\label{lemma:caratterizzazionecircuiti0n}
  For all $c\in \Diag{\SigPB}[1,A^n]$, either $c\eqPB \Flipn{\bot}$ or $c\eqPB b$ for some $b\in \Diag{\SigB}[1,A^n]$.
\end{lemma}


\subsection{Probabilistic Boolean circuits}\label{ssec:probabilisticboolean}
Finally, we illustrate probabilistic Boolean circuits from \cite{piedeleu2025boolean}.
%
Consider the monoidal signature  \[ \SigPRB \defeq \SigPB \cup\{ \Flip{p} \mid p\in (0,1)\}\]  
 where $\Flip{p}$ denotes a probabilistic gate that receives no input and emits a Boolean signal on the right, which is $1$ with probability $p$ and $0$ with probability $1-p$. Thus, string diagrams in $\Diag{\SigPRB}$ represent arrows of $\KlD$, the Kleisli category of the subdistributions monad $\subdistr\colon \Sets \to \Sets$ (see e.g.,~\cite{hasuo2007generic}), which assigns to every set $X$ the set of \emph{subdistributions} over  $X$, i.e.\ the set of functions $d\colon X\to [0,1]$  such that $\sum_{x\in X}d(x)\leq 1$, and $d(x)\neq 0$ for only finitely many $x\in X$. 
 
 
 Recall that objects of $\KlD$ are sets; morphisms \(f \colon X \to Y\) are functions \(X \to \subdistr(Y)\). 
  We often write \(f(y \mid x)\) for \(f(x)(y)\), as this number represents the probability that \(f\) returns \(y\) given the input \(x\).
  Identities \(\id{X} \colon X \to \subdistr(X)\) map each element \(x \in X\) to \(\delta_{x}\).
  For two functions \(f \colon X \to \subdistr(Y)\) and \(g \colon Y \to \subdistr(Z)\), their composition in $\KlD$ is defined as \(f ; g (z \mid x) \defeq \sum_{y \in Y} f(y \mid x) \cdot g(z \mid y)\).


To formally define their semantics, consider the symmetric monoidal structure $(\KlD, \otimes, \uno)$, where $\otimes$ is the cartesian product of sets with unit the singleton $\uno \defeq \{\bullet\}$ and, for arrows  \(f \colon X \to Y\) and \(g \colon X' \to Y'\), $f\per g\colon X\otimes X' \to Y \otimes Y'$ is defined, for all $x\in X$, $x'\in X'$, $y\in Y$, $y'\in Y'$, as follows.
\begin{equation}\label{ex:products}
\begin{aligned}
f \per g(y,y' \mid x,x') &\defeq f(y \mid x) \cdot g(y' \mid x')
\end{aligned}
\end{equation}
And observe that there is an obvious monoidal embedding $\ParJ\colon \Cat{Par} \to \KlD$ which is the identity on objects and associates to a partial function $f\colon X \to Y$ the function $\ParJ(f)\colon X \to \Dis(Y)$, mapping $x$ to $\delta_{f(x)}$, if $f(x)$ is defined and to the null distribution $\star$ otherwise. 




The semantics of $\SigPRB$ is given by the monoidal functor $\osem{-}\colon \Diag{\SigPRB} \to \KlD$ defined on objects as $A^n \mapsto 2^n$. On arrows, it is defined by first interpreting generators  $c\in \SigPB$ as $\ParJ(\osemPB{c})$, i.e.
\[
    \begin{array}{rclrclrcl}
      \osem{\Andgate}\colon 2 \times 2& \to & 2  & \osem{\Notgate}\colon  2& \to & 2 & \osem{\Flip{1}} \colon 1 & \to & 2 \\
      (x,y)&\mapsto&\delta_{x\wedge y} &  x & \mapsto & \delta_{\neg x} & \bullet &\mapsto&\delta_{1}\\[4pt]
       \osem{\CBcopier} \colon 2  & \to & 2\times 2 & \osem{\CBdischarger} \colon 2 & \to & 1 & \osem{\CBcocopier} \colon 2 \times 2 & \to & 2  \\
      x &\mapsto&\delta_{(x,x)} & x &\mapsto&\delta_{\bullet} & (x,y) &\mapsto& \begin{cases}\delta_{x} &\text{if }x=y\\ \star & \text{else}\end{cases}, 
    \end{array}
  \]

 the generator $\Flip{p}$ as 
\begin{equation}\label{eq:semanticsFlip}
\begin{array}{rcl}
      \osem{\Flip{p}}\colon 1& \to & 2   \\
      \bullet&\mapsto& \delta_1 +_p \delta_0  \end{array}
    \end{equation}
and then inductively on the structure of the monoidal category $(\KlD, \otimes, \uno)$. Simple computations confirm that $\osem{-}$ extends both $\osemB{-}$ and $\osemPB{-}$, in the sense that the following diagrams commute.
\[
\xymatrix{\Diag{\SigB} \ar@{^{(}->}[r] \ar[d]_{\osemB{-}}& \Diag{\SigPB} \ar@{^{(}->}[r] \ar[d]|{\osemPB{-}} & \Diag{\SigPRB} \ar[d]^{\osem{-}}\\
\Sets \ar@{^{(}->}[r]_{\Pa}& \Cat{Par} \ar@{^{(}->}[r]_{\ParJ}& \KlD
}
\]








\medskip
Figures~4 and~5 in \cite{piedeleu2025boolean} provide a sound and complete equational axiomatisation of probabilistic Boolean circuits. The system essentially consists of the axioms of Boolean algebras (reported in Figure~\ref{tab:booleanalgebra}), together with four non-trivial axioms governing the behaviour of $\Flip{p}$ and additional axioms for $\CBcocopier$, which differ from those presented in Figure~\ref{tab:partialbooleanalgebra}.

Importantly, the equivalence induced by these axioms is strictly coarser than the one given by $\osem{-}$. In fact, two diagrams $c$ and $d$ are equivalent under the axioms of \cite{piedeleu2025boolean} if and only if $\osem{c} \propto \osem{d}$. The relation $\propto$ is defined on arrows of $\KlD$ by setting $f \propto g$ whenever there exists a real number $\lambda > 0$ such that $f(y\mid x) = \lambda \cdot g(y\mid x)$ for all $x \in X$ and $y \in Y$. %In the next section, we provide a complete  axiomatisation for the equivalence induced by $\osem{-}$ by means of probabilistic tape diagrams.





==> sections/probabilisticbooleantapes-NEW.tex <==
\section{Completeness for Probabilistic Boolean Tapes}\label{sec:completenessprobbooltapes-NEW}
 \marginpar{C: $\tapeeqPB$ è in appendice. nel testo principale possiamo farne a meno e risparmiare spazio. }
 


 
 
 
Before proceeding, it is convenient to consider also the category $ \CatT{\Diag{\ThPB}}$ of tape diagrams generated by the quotient theory $\ThPB$. Its description is the same as $\CatT{\Diag{\SigPB}}$ of Section~\ref{sec:encodingprobboolcircuits}, but string diagrams are quotiented by $\eqPB$. The functor $\CatT{Q_\ThPB} \colon \CatT{\Diag{\SigPB}} \to \CatT{\Diag{\ThPB}}$
obtained by applying the functor $\CatT{-}$ to $Q_\ThPB\colon \Diag{\SigPB} \to \Diag{\ThPB}$, namely the symmetric monoidal functor mapping each string diagram into its $=_{\ThPB}$-equivalence class.  

\subsection{Axiomatisation}\label{ssec:probbooltapes:axiomatisation}
In order to provide a complete axiomatisation for the equivalence induced by $\dsem{-}$, we reuse $\eqPB$ which, as proved in Theorem \ref{thm:completenesspartialcircuits}, provides a complete axiomatisation for partial Boolean circuits. 
Since the axioms in $\ThPB$ are sound with respect to $\osem{-}$ and since $\osem{-}=\dsem{\encoding{-}}$, these axioms are also sound for $\dsem{-}$. However, they are not complete, as explained below.

\begin{example}
Consider $ \CatT{\Diag{\ThPB}}$ which, 
by Corollary~\ref{cor:isotapematrices} and Proposition~\ref{prop:isopartialboolean} is isomorphic to $\stmat{\Cat{Par}_2^+}$. Now consider only $1\times 1$ matrices: these are arrows in $\Cat{Par}_2^+$, i.e., subdistributions of partial functions. These are not in one-to-one correspondence with Kleisli arrows. Take for instance the null subdistribution $\star \in \Dis(\Cat{Par}[1, 2])$ and $\delta_\bot \in \Dis(\Cat{Par}[1, 2])$ which are distinct arrows in $\Cat{Par}_2^+[1,2]$. The former is drawn as the tape \scalebox{0.6}{\tikzfig{tapes/cipriano/AXPBP2right}} and the latter as $\Flip{\bot}[t]$. It is easy to see that $\dsem{-}$ maps both diagrams into the $\KlD$-arrow $\star_{1,2}$.
\end{example}



To obtain a complete axiomatisation, we need to add to $\ThPB$ the axioms in Figure~\ref{ax:BooleanTAPES}. The tape diagram on the right-hand side of \eqref{ax:AXPBP1} with probability $\frac{1}{2}$ tests if the input is $1$ and returns $1$ and, with probability $\frac{1}{2}$, tests if the input is $0$ and returns $0$. The equality \eqref{ax:AXPBP1} forces such tape to be equal to $\frac{1}{2} \cdot \id{A}$; Axiom \eqref{ax:AXPBP2} forces $\Flip{\bot}[t]$ to be the null subdistribution; Axiom \eqref{ax:canc} is an implication which asserts cancellativity: see Section~\ref{sub:sec:preliminaries:pca}. 



\begin{figure}[H]
  \centering

  \mylabelbis{ax:AXPBP1}{T2}
  \mylabelbis{ax:AXPBP2}{T1}
  \mylabelbis{ax:canc}{T3}

  \[
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}ccc@{}}
    \scalebox{0.90}{$
      \tikzfig{tapes/cipriano/AXPBP2left}
      \stackrel{\eqref{ax:AXPBP2}}{=}
      \tikzfig{tapes/cipriano/AXPBP2right}
    $}
    &
    \scalebox{0.80}{$
      \tikzfig{tapes/cipriano/AXPBP1left}
      \stackrel{\eqref{ax:AXPBP1}}{=}
      \tikzfig{tapes/cipriano/AXPBP1right}
    $}
    &
    \scalebox{0.80}{$
      \tikzfig{tapes/cipriano/Axcancleft}
      \stackrel{\eqref{ax:canc}}{\implies}
      \tikzfig{tapes/cipriano/Axcancright}
    $}
  \end{tabular*}
  \]

  \caption{Axioms for tapes of partial Boolean circuits.}
  \label{ax:BooleanTAPES}
\end{figure}

From $\ThPB$ and the axioms in Figure~\ref{ax:BooleanTAPES}, one generates the congruence $\dot{\sim}$ on $\CatT{\Diag{\SigPB}}$ by means of the following inference rules.
\begin{equation}\label{eq:congr3}
        \scalebox{0.85}{$
        \centering
        \begin{array}{c}
        \begin{array}{c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c}
            \inferrule*[right=\eqref{ax:AXPBP1}]{\t_1 \stackrel{\eqref{ax:AXPBP1}}{=} \t_2}{\t_1 \dot{\sim} \t_2}
            &
            \inferrule*[right=\eqref{ax:AXPBP2}]{\t_1 \stackrel{\eqref{ax:AXPBP2}}{=} \t_2}{\t_1 \dot{\sim} \t_2}
            &
            \inferrule*[right=($\textsc{R}$)]{-}{\t \dot{\sim} \t}
            &
            \inferrule*[right=($\textsc{S}$)]{\t_1 \dot{\sim} \t_2}{\t_2 \dot{\sim} \t_1}
            &    
            \inferrule*[right=($\textsc{T}$)]{\t_1 \dot{\sim} \t_2 \quad \t_2 \dot{\sim} \t_3}{\t_1 \dot{\sim} \t_3}
            % &
            % \inferrule*[right=($E$)]{ (t,t') \in E \and U \in \sort^\star}{ t_U \dot{\sim} t'_U}
        \end{array}
        \\[10pt]
        \begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c@{\qquad}c}
        \inferrule*[right=($\ThPB$)]{c \eqPB d}{\tape{c} \dot{\sim} \tape{d}}
            &
            \inferrule*[right=\eqref{ax:canc}]{p\cdot \t \dot{\sim} p\cdot \s }{\t \dot{\sim} \s}
            &
            \inferrule*[right=($;$)]{\t_1 \dot{\sim} \t_2 \quad \s_1 \dot{\sim} \s_2}{\t_1;\s_1 \dot{\sim} \t_2;\s_2}
            &
            \inferrule*[right=($\piu$)]{\t_1 \dot{\sim} \t_2 \quad \s_1 \dot{\sim} \s_2}{\t_1\piu\s_1 \dot{\sim} \t_2 \piu \s_2}
            &
            \inferrule*[right=($\per $)]{\t_1 \dot{\sim} \t_2 \quad \s_1 \dot{\sim} \s_2}{\t_1\per \s_1 \dot{\sim} \t_2 \per \s_2}       
        \end{array}
        \end{array}
        $}
\end{equation}

Simple computations confirm that the axioms are sound.
\begin{proposition}[Soundness]\label{prop:soundnesstapes}
For all $\s,\t \in \CatT{\Diag{\SigPB}}$, if $\s \eqsynbis \t$ then $\dsem{\s}=\dsem{\t}$.
\end{proposition}


To prove completeness, it is convenient to consider diagrams in $\CatT{\Diag{\ThPB}}$. Let $\eqsyn$ be the congruence on $\CatT{\Diag{\ThPB}}$ defined as $\dot{\sim}$ but omitting the rule ($\ThPB$). 


\begin{proposition}\label{prop:twoequivalence}
For all $\s , \t \in \CatT{\Diag{\SigPB}}$, $\s \dot{\sim} \t$ iff $\CatT{Q_{\ThPB}}(\s) \eqsyn \CatT{Q_{\ThPB}}(\t)$.
\end{proposition}




Thanks to the above proposition, we can work with $\eqsyn$ rather than $\dot{\sim}$. We conclude this section by illustrating three key properties of $\eqsyn$. First, axiom \eqref{ax:AXPBP2} easily entails the following.

\begin{lemma}\label{lemma:bottomstar2}
%\label{axpbp2m}
 $\star_{A^0,A^n} \sim \Flipn{\bot}[t]$.  
\end{lemma}


Hereafter, we write $\Cat{B}[1,A^n]$ for the set of $n$-ary Boolean vectors, i.e., all those tapes in $\CatT{\Diag{\ThPB}}[1,A^n]$ of the form $\overrightarrow{b}\defeq\bigotimes_{i=1}^n b_i$ for $b_i \in \{\Flip{0}[t], \Flip{1}[t]\}$ if $n\not=0$, and $\tikzfig{tapes/empty}$ if $n=0$. If $\overrightarrow{b}\in\Cat{B}[1,A^n]$, we write $\overleftarrow{b}$ for the tape $\bigotimes_{i=1}^n b'_i\in \CatT{\Diag{\ThPB}}[A^n,1]$ where $b'_i$ is $\coflip{1}[t]$ if $b_i$ is $\Flip{1}[t]$ and $\coflip{0}[t]$ if $b_i$ is $\Flip{0}[t]$.

The second property crucially relies on axiom \eqref{ax:AXPBP1} and on the monoidal enrichment of $\CatT{\Diag{\ThPB}}$ over $\Cat{PCA}$ (see \cite[Thm.\ 27]{bonchi2025tapediagramsmonoidalmonads}), i.e., for all $p\in(0,1)$ and properly typed $\t,\s_1,\s_2$:
\begin{equation}\label{eq:monoidalenrichment} \t \otimes (\s_1+_p \s_2)= (\t \otimes \s_1)+_p(\t \otimes \s_2) \qquad  (\s_1+_p \s_2)  \otimes \t= ( \s_1 \otimes \t )+_p(\s_2 \otimes  \t) \qquad \star \otimes\, \t= \star = \t\otimes \star \end{equation}

\begin{lemma}\label{lemma:axiomsninput}
%\label{axpbp1m}
 For all $n\in \mathbb{N}$, $\frac{1}{2^n}\cdot \id{A^n} \sim \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b}$;
\end{lemma}


The  lemma above and axiom \eqref{ax:canc} give us the third key result.

\begin{lemma}\label{lemma:PBP2} 
Let $\s,\t\in \CatT{\Diag{\ThPB}}[A^n,A^m]$. If, for all $\overrightarrow{b}\in \Cat{B}[1,A^n]$, $\overrightarrow{b};\s \eqsyn\overrightarrow{b}; \t$, then $\s \eqsyn \t$.
\end{lemma}



\subsection{Completeness}\label{ssec:probbooltapes:completeness}
We denote with $\eqsynq{\CatT{\Diag{\ThPB}}}$ for the quotient of $\CatT{\Diag{\ThPB}}$ with $\eqsyn$ and by $Q_\eqsyn\colon \CatT{\Diag{\ThPB}} \to \eqsynq{\CatT{\Diag{\ThPB}}}$ the functor mapping each tape into its $\eqsyn$ equivalence class. By Propositions~\ref{prop:soundnesstapes} and \ref{prop:twoequivalence}, $\dsem{-}\colon \CatT{\Diag{\SigPB}} \to \KlD$ can be factored as
\[\xymatrix{\CatT{\Diag{\SigPB}} \ar[r]^{\CatT{Q_\ThPB}} & \CatT{\Diag{\ThPB}} \ar[r]^{Q_\eqsyn} & \eqsynq{\CatT{\Diag{\ThPB}}} \ar@{.>}[r]^I& \KlD}\]
for some functor $I$. Proving completeness amounts to proving that  $I$  is faithful. %\colon \eqsynq{\CatT{\Diag{BPar}}} \to \KlD$

\medskip


%By Corollary~\ref{cor:isotapematrices} and Proposition~\ref{prop:isopartialboolean}  we know that \[\CatT{\Diag{\ThPB}} \cong \stmat{\Diag{\ThPB}^+}\cong \stmat{\Cat{Par}_2^+}\text{.}\] 
%
 Now, %let $\KlD_2$ be the full subcategory of $\KlD$ having as objects the sets $2^n$ for all $n\in \mathbb{N}$,
%and 
observe that $\ParJ\colon \,\Cat{Par} \to \KlD$ from Section~\ref{ssec:partialboolean} restricts to $\ParJ_2\colon \Cat{Par}_2 \to \KlD$. Since $\KlD$ is a convex biproduct category, by the two adjunctions in \eqref{eq:adjunctions}, there exists a functor \[\ParJ_2'\colon \stmat{\Cat{Par}_2^+} \to \KlD\text{.} \]

Hence, consider the following diagram where the left vertical isomorphisms are given by Corollary~\ref{cor:isotapematrices} and Proposition~\ref{prop:isopartialboolean}.
%\[\xymatrix{
%\CatT{\Diag{\ThPB}}  \ar[r]^{\eqsynq{Q}} \ar[d]_{i} & \eqsynq{\CatT{\Diag{\ThPB}}} \ar[d]^{I}  \\
%\stmat{\Cat{Par}_2^+} \ar[r]_{\ParJ_2'} & \KlD
%}\]
\[
\xymatrix@R=2ex@C=3ex{
\CatT{\Diag{\ThPB}} \ar[r]^{\eqsynq{Q}} \ar[d]_{\cong} 
  & \eqsynq{\CatT{\Diag{\ThPB}}} \ar[dd]^{I} \\
{\stmat{\Diag{\ThPB}^+}} \ar[d]_{\cong} 
  & {} \\
\stmat{\Cat{Par}_2^+} \ar[r]_{\ParJ_2'} 
  & \KlD
}
\]
Denoted with $\iso$ the composition of left vertical arrows, we obtain the following result.
\begin{lemma}\label{lemma:diagramma-commutativo}
  The above diagram commutes, i.e., $I\circ \eqsynq{Q}=\ParJ_2'\circ \iso$.
\end{lemma}



 In order to prove that $I$ is faithful, we first prove some useful lemmas.


\begin{lemma}\label{lemma:Ffaith}
For all $\t,\t'\in \CatT{\Diag{\ThB}}[A^0,A^m]$, if $\ParJ_2'\circ \iso(\t)=\ParJ_2'\circ \iso(\t')$, then $\t=\t'$.
\end{lemma}



Now, by relying on Lemma~\ref{lemma:caratterizzazionecircuiti0n}, we have the following normal forms for tapes $\t \colon A^0 \to A^m$.

\begin{lemma}\label{lemma:PBP0}
For all  $\t\in \CatT{\Diag{\ThPB}}[A^0,A^m]$, there exist, for  $i=1,\dots,n$,  $p_i\in (0,1)$ such that $\sum_{i=1}^{n}p_i= 1$, $\overrightarrow{b}_i\in \Cat{B}[1,A^m]$ and $p,q\in [0,1]$ such that $$\t=(\sum_{i=1}^{n}p_i\cdot \overrightarrow{b}_i)+_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t])\text{.}$$ 
  \end{lemma}


The previous two results, combined with Lemma~\ref{lemma:bottomstar2} allow us to prove the following key property.

\begin{lemma}\label{lemma:PBP1}
  For all $\t,\t'\in \CatT{\Diag{\ThPB}}[A^0,A^m]$, if $\ParJ_2'\circ \iso(\t)=\ParJ_2'\circ \iso(\t')$, then $\t\sim \t'$.
\end{lemma}





\begin{theorem}\label{thm:completenessPBPtapes}
  $I\colon \eqsynq{\CatT{\Diag{\ThPB}}} \to \stmat{\KlD_2}$ is faithful.%\marginpar{Il Codminio di $H$ e' sbagliato}
\end{theorem}
\begin{proof}
  Let $[\t]_\sim, [\s]_\sim \in \eqsynq{\CatT{\Diag{\ThPB}}}[A^n,A^m]$ be such that $I([\t]_\sim)=I([\s]_\sim)$. Then, consider the following derivation:
  \begin{align}
    I([\t]_\sim)=I([\s]_\sim) &\implies \ParJ_2'\circ \iso(\t)=\ParJ_2'\circ \iso(\s) \tag{Lemma \ref{lemma:diagramma-commutativo}}\\
    &\implies \text{for all } b\in \Cat{B}[1,A^n], \ParJ_2' (\iso(b));\ParJ_2'( \iso(\t))=\ParJ_2'(\iso(b));\ParJ_2' (\iso(\s) )\notag \\
    &\implies \text{for all } b\in \Cat{B}[1,A^n], \ParJ_2'\circ \iso(b;\t)=\ParJ_2'\circ \iso(b;\s) \tag{Functoriality}\\
    &\implies \text{for all } b\in \Cat{B}[1,A^n], b;\t \eqsyn b;\s \tag{Lemma \ref{lemma:PBP1}}\\
    &\implies \t \eqsyn \s \tag{Lemma \ref{lemma:PBP2}}
  \end{align}
  Hence, $[\t]_\sim=[\s]_\sim$. The above derivation proves that $I$ is faithful for arrows of type $A^n \to A^m$. For arrows of type $ A^k \to \bigoplus_{i=1}^nA^{m_i}$ one can rely on convex products and reduce to the previous case. While for arrows of arbitrary type $\bigoplus_{j=1}^o A^{k_j} \to \bigoplus_{i=1}^nA^{m_i}$, one can easily rely on the universal property of coproducts, see Appendix~\ref{app:{sec:completenessprobbooltapes-NEW}}
 for more details.
\end{proof}







\begin{corollary}[Completeness]\label{cor:completenessPBPtapes}
  For all $\s,\t \in \CatT{\Diag{\SigPB}}$, if $\dsem{\s}=\dsem{\t}$ then $\s \eqsynbis \t$.
\end{corollary}

\begin{proof}[Proof of Corollary~\ref{cor:completenessPBPtapes}]
By Theorem~\ref{thm:completenessPBPtapes}, $I$ is faithful. The following derivation concludes the proof.
  \begin{align}
    \dsem{\s}=\dsem{\t} &\Longleftrightarrow (\CatT{Q_{\ThPB}}; Q_\eqsyn ; I) (\s)= (\CatT{Q_{\ThPB}}; Q_\eqsyn ; I) (\t) \tag{$\dsem{-}= \CatT{Q_{\ThPB}}; Q_\eqsyn ; I$}\\
    &\implies   (\CatT{Q_{\ThPB}}; Q_\eqsyn ) (\s)= (\CatT{Q_{\ThPB}}; Q_\eqsyn )(\t) \tag{$I$ is faithful} \\
    &\Longleftrightarrow \CatT{Q_{\ThPB}}  (\s) \eqsyn \CatT{Q_{\ThPB}}(\t) \tag{Def. $Q_\eqsyn$}\\
    &\Longleftrightarrow \s \dot{\sim} \t \tag{Proposition \ref{prop:twoequivalence}}
  \end{align}
\end{proof}


\begin{corollary}\label{cor:finale}
  For all $c,d \in \Diag{\SigPRB}$, $\osem{c}=\osem{d}$ iff $\encoding{c} \eqsynbis \encoding{d}$.
\end{corollary}
%
\begin{proof}[Proof of Corollary \ref{cor:finale}]
  \begin{align}
    \osem{c}=\osem{d} &\Longleftrightarrow  \dsem{\encoding{c}}=\dsem{\encoding{c}} \tag{Proposition \ref{prop:encoding}}\\
    &\Longleftrightarrow \encoding{c} \eqsynbis \encoding{d} \tag{Proposition \ref{prop:soundnesstapes}, Corollary \ref{cor:completenessPBPtapes}}
  \end{align}
\end{proof}



==> sections/probabilisticbooleantapes.tex <==
\section{Completeness for Probabilistic Boolean Tapes}\label{sec:completenessprobbooltapes}
 \marginpar{C: $\tapeeqPB$ è in appendice. nel testo principale possiamo farne a meno e risparmiare spazio. }
Before proceeding, it is convenient to consider also the category $ \CatT{\Diag{\ThPB}}$ of tape diagrams generated by the quotient theory $\ThPB$. Its description is the same as $\CatT{\Diag{\SigPB}}$ of Section~\ref{sec:encodingprobboolcircuits}, but string diagrams are quotiented by $\eqPB$. The functor $\CatT{Q_\ThPB} \colon \CatT{\Diag{\SigPB}} \to \CatT{\Diag{\ThPB}}$
obtained by applying the functor $\CatT{-}$ to $Q_\ThPB\colon \Diag{\SigPB} \to \Diag{\ThPB}$, namely the symmetric monoidal functor mapping each string diagram into its $=_{\ThPB}$-equivalence class.  

\subsection{Axiomatisation}\label{ssec:probbooltapes:axiomatisation}
In order to provide a complete axiomatisation for the equivalence induced by $\dsem{-}$, we reuse $\eqPB$ which, as proved in Theorem \ref{thm:completenesspartialcircuits}, provides a complete axiomatisation for partial Boolean circuits. 
Since the axioms in $\ThPB$ are sound with respect to $\osem{-}$ and since $\osem{-}=\dsem{\encoding{-}}$, these axioms are also sound for $\dsem{-}$. However, they are not complete, as explained below.

\begin{example}
Consider $ \CatT{\Diag{\ThPB}}$ which, 
by Corollary~\ref{cor:isotapematrices} and Proposition~\ref{prop:isopartialboolean} is isomorphic to $\stmat{\Cat{Par}_2^+}$. Now consider only $1\times 1$ matrices: these are arrows in $\Cat{Par}_2^+$, i.e., subdistributions of partial functions. These are not in one-to-one correspondence with Kleisli arrows. Take for instance the null subdistribution $\star \in \Dis(\Cat{Par}[1, 2])$ and $\delta_\bot \in \Dis(\Cat{Par}[1, 2])$ which are distinct arrows in $\Cat{Par}_2^+[1,2]$. The former is drawn as the tape \scalebox{0.6}{\tikzfig{tapes/cipriano/AXPBP2right}} and the latter as $\Flip{\bot}[t]$. It is easy to see that $\dsem{-}$ maps both diagrams into the $\KlD$-arrow $\star_{1,2}$.
\end{example}



To obtain a complete axiomatisation, we need to add to $\ThPB$ the axioms in Figure~\ref{ax:BooleanTAPES}. The tape diagram on the right-hand side of \eqref{ax:AXPBP1} with probability $\frac{1}{2}$ tests if the input is $1$ and returns $1$ and, with probability $\frac{1}{2}$, tests if the input is $0$ and returns $0$. The equality \eqref{ax:AXPBP1} forces such tape to be equal to $\frac{1}{2} \cdot \id{A}$; Axiom \eqref{ax:AXPBP2} forces $\Flip{\bot}[t]$ to be the null subdistribution; Axiom \eqref{ax:canc} is an implication which asserts cancellativity: see Section~\ref{sub:sec:preliminaries:pca}. 

\begin{figure}[H]
  \centering

  % Labels
  \mylabelbis{ax:AXPBP1}{T1}
  \mylabelbis{ax:AXPBP2}{T2}
  \mylabelbis{ax:canc}{T3}

  \[
  \begin{array}{c@{\quad}c@{\quad}c}
    % Primo assioma (ridotto)
    \scalebox{0.80}{$
      \tikzfig{tapes/cipriano/AXPBP1left}
      \stackrel{\eqref{ax:AXPBP1}}{=}
      \tikzfig{tapes/cipriano/AXPBP1right}
    $}
    &
    % Secondo assioma (normale)
    \scalebox{0.90}{$
      \tikzfig{tapes/cipriano/AXPBP2left}
      \stackrel{\eqref{ax:AXPBP2}}{=}
      \tikzfig{tapes/cipriano/AXPBP2right}
    $}
    &
    % Terzo assioma (più piccolo)
    \scalebox{0.80}{$
      \tikzfig{tapes/cipriano/Axcancleft}
      \stackrel{\eqref{ax:canc}}{\implies}
      \tikzfig{tapes/cipriano/Axcancright}
    $}
  \end{array}
  \]

  \caption{Axioms for tapes of partial Boolean circuits.}
  \label{ax:BooleanTAPES}
\end{figure}

From $\ThPB$ and the axioms in Figure~\ref{ax:BooleanTAPES}, one generates the congruence $\dot{\sim}$ on $\CatT{\Diag{\SigPB}}$ by means of the following inference rules.
\begin{equation}\label{eq:congr3}
        \scalebox{0.85}{$
        \centering
        \begin{array}{c}
        \begin{array}{c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c}
            \inferrule*[right=\eqref{ax:AXPBP1}]{\t_1 \stackrel{\eqref{ax:AXPBP1}}{=} \t_2}{\t_1 \dot{\sim} \t_2}
            &
            \inferrule*[right=\eqref{ax:AXPBP2}]{\t_1 \stackrel{\eqref{ax:AXPBP2}}{=} \t_2}{\t_1 \dot{\sim} \t_2}
            &
            \inferrule*[right=($\textsc{R}$)]{-}{\t \dot{\sim} \t}
            &
            \inferrule*[right=($\textsc{S}$)]{\t_1 \dot{\sim} \t_2}{\t_2 \dot{\sim} \t_1}
            &    
            \inferrule*[right=($\textsc{T}$)]{\t_1 \dot{\sim} \t_2 \quad \t_2 \dot{\sim} \t_3}{\t_1 \dot{\sim} \t_3}
            % &
            % \inferrule*[right=($E$)]{ (t,t') \in E \and U \in \sort^\star}{ t_U \dot{\sim} t'_U}
        \end{array}
        \\[10pt]
        \begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c@{\qquad}c}
        \inferrule*[right=($\ThPB$)]{c \eqPB d}{\tape{c} \dot{\sim} \tape{d}}
            &
            \inferrule*[right=\eqref{ax:canc}]{p\cdot \t \dot{\sim} p\cdot \s }{\t \dot{\sim} \s}
            &
            \inferrule*[right=($;$)]{\t_1 \dot{\sim} \t_2 \quad \s_1 \dot{\sim} \s_2}{\t_1;\s_1 \dot{\sim} \t_2;\s_2}
            &
            \inferrule*[right=($\piu$)]{\t_1 \dot{\sim} \t_2 \quad \s_1 \dot{\sim} \s_2}{\t_1\piu\s_1 \dot{\sim} \t_2 \piu \s_2}
            &
            \inferrule*[right=($\per $)]{\t_1 \dot{\sim} \t_2 \quad \s_1 \dot{\sim} \s_2}{\t_1\per \s_1 \dot{\sim} \t_2 \per \s_2}       
        \end{array}
        \end{array}
        $}
\end{equation}

Simple computations confirm that the axioms are sound.
\begin{proposition}[Soundness]\label{prop:soundnesstapes}
For all $\s,\t \in \CatT{\Diag{\SigPB}}$, if $\s \eqsynbis \t$ then $\dsem{\s}=\dsem{\t}$.
\end{proposition}


To prove completeness, it is convenient to consider diagrams in $\CatT{\Diag{\ThPB}}$. Let $\eqsyn$ be the congruence on $\CatT{\Diag{\ThPB}}$ defined as $\dot{\sim}$ but omitting the rule ($\ThPB$). 


\begin{proposition}\label{prop:twoequivalence}
For all $\s , \t \in \CatT{\Diag{\SigPB}}$, $\s \dot{\sim} \t$ iff $\CatT{Q_{\ThPB}}(\s) \eqsyn \CatT{Q_{\ThPB}}(\t)$.
\end{proposition}




Thanks to the above proposition, we can work with $\eqsyn$ rather than $\dot{\sim}$. We conclude this section by illustrating three key properties of $\eqsyn$. First, axiom \eqref{ax:AXPBP2} easily entails the following.

\begin{lemma}\label{lemma:bottomstar2}
%\label{axpbp2m}
 $\star_{A^0,A^n} \sim \Flipn{\bot}[t]$.  
\end{lemma}


Hereafter, we write $\Cat{B}[1,A^n]$ for the set of $n$-ary Boolean vectors, i.e., all those tapes in $\CatT{\Diag{\ThPB}}[1,A^n]$ of the form $\overrightarrow{b}\defeq\bigotimes_{i=1}^n b_i$ for $b_i \in \{\Flip{0}[t], \Flip{1}[t]\}$ if $n\not=0$, and $\tikzfig{tapes/empty}$ if $n=0$. If $\overrightarrow{b}\in\Cat{B}[1,A^n]$, we write $\overleftarrow{b}$ for the tape $\bigotimes_{i=1}^n b'_i\in \CatT{\Diag{\ThPB}}[A^n,1]$ where $b'_i$ is $\coflip{1}[t]$ if $b_i$ is $\Flip{1}[t]$ and $\coflip{0}[t]$ if $b_i$ is $\Flip{0}[t]$.

The second property crucially relies on axiom \eqref{ax:AXPBP1} and on the monoidal enrichment of $\CatT{\Diag{\ThPB}}$ over $\Cat{PCA}$ (see \cite[Thm.\ 27]{bonchi2025tapediagramsmonoidalmonads}), i.e., for all $p\in(0,1)$ and properly typed $\t,\s_1,\s_2$:
\begin{equation}\label{eq:monoidalenrichment} \t \otimes (\s_1+_p \s_2)= (\t \otimes \s_1)+_p(\t \otimes \s_2) \qquad  (\s_1+_p \s_2)  \otimes \t= ( \s_1 \otimes \t )+_p(\s_2 \otimes  \t) \qquad \star \otimes\, \t= \star = \t\otimes \star \end{equation}

\begin{lemma}\label{lemma:axiomsninput}
%\label{axpbp1m}
 For all $n\in \mathbb{N}$, $\frac{1}{2^n}\cdot \id{A^n} \sim \sum_{\overrightarrow{b}\in \Cat{B}[1,A^n]}^{} \frac{1}{2^n}\cdot\overleftarrow{b};\overrightarrow{b}$;
\end{lemma}


The  lemma above and axiom \eqref{ax:canc} give us the third key result.

\begin{lemma}\label{lemma:PBP2} 
Let $\s,\t\in \CatT{\Diag{\ThPB}}[A^n,A^m]$. If, for all $\overrightarrow{b}\in \Cat{B}[1,A^n]$, $\overrightarrow{b};\s \eqsyn\overrightarrow{b}; \t$, then $\s \eqsyn \t$.
\end{lemma}



\subsection{Completeness}\label{ssec:probbooltapes:completeness}
We write $\eqsynq{\CatT{\Diag{\ThPB}}}$ for the category obtained as the quotient of $\CatT{\Diag{\ThPB}}$ by $\eqsyn$ and by $Q_\eqsyn\colon \CatT{\Diag{\ThPB}} \to \eqsynq{\CatT{\Diag{\ThPB}}}$ the functor mapping each tape into its $\eqsyn$ equivalence class. By Propositions~\ref{prop:soundnesstapes} and \ref{prop:twoequivalence}, $\dsem{-}\colon \CatT{\Diag{\SigPB}} \to \KlD$ can be factored as
\[\xymatrix{\CatT{\Diag{\SigPB}} \ar[r]^{\CatT{Q_\ThPB}} & \CatT{\Diag{\ThPB}} \ar[r]^{Q_\eqsyn} & \eqsynq{\CatT{\Diag{\ThPB}}} \ar@{.>}[r]^I& \KlD}\]
for some functor $I$. Proving completeness amounts to proving that  $I$  is faithful. %\colon \eqsynq{\CatT{\Diag{BPar}}} \to \KlD$

\medskip

%\marginpar{C:Quando diciamo che J=P;ParJ? inoltre non dovrebbe andare da Set?}
By Corollary~\ref{cor:isotapematrices} and Proposition~\ref{prop:isopartialboolean}  we know that \[\CatT{\Diag{\ThPB}} \cong \stmat{\Diag{\ThPB}^+}\cong \stmat{\Cat{Par}_2^+}\text{.}\] 
%
Now, let $\KlD_2$ be the full subcategory of $\KlD$ having as objects the sets $2^n$ for all $n\in \mathbb{N}$,
and observe that the functor $\ParJ\colon \,\mathrm{Par}(\Sets) \to \KlD$ from Section~\ref{ssec:partialboolean} restricts and corestricts to $\ParJ_2\colon \Cat{Par}_2 \to \KlD_2$. Since $\KlD_2$ is $\Cat{PCA}$-enriched, by Theorem~\ref{thm:freeenriched}, there exists \[\ParJ_2^\sharp\colon \Cat{Par}_2^+ \to \KlD_2\text{.}\]


We call $F\colon \CatT{\Diag{\ThPB}} \to \stmat{\KlD_2}$, the morphism of convex biproduct categories obtained by composing the isomorphism $\CatT{\Diag{\ThPB}} \to  \stmat{\Cat{Par}_2^+}$ followed by $\stmat{\ParJ^\sharp}$. 
%\marginpar{C: prova di dimostrazione che fa a meno di $\J$.}

We call $G\colon \stmat{\KlD_2} \to \KlD$ the morphism of convex biproduct categories obtained by composing the embedding $\stmat{\KlD_2} \to \stmat{\KlD}$ with the counit of the adjunction in Theorem~\ref{thm:matfree}, $\epsilon_{\KlD} \colon \stmat{\KlD}\to \KlD$. The latter is, by Theorem~\ref{thm:matfree}, full and faithful and, therefore, so is $G$. 
\[\xymatrix{
\CatT{\Diag{\ThPB}}  \ar[r]^{\eqsynq{Q}} \ar[d]_{F} & \eqsynq{\CatT{\Diag{\ThPB}}} \ar[d]^{I} \ar@{.>}[dl]|H \\
\stmat{\KlD_2} \ar[r]_G & \KlD
}\]
%
\begin{comment}
We recall from \cite{arxivprobbooltapes} the following property of $\J^\sharp$.
\begin{lemma}\label{lemma:Jfaithful}
For all $d_1,d_2\in \Sets_2^+[1, 2^m]$, $\J^\sharp(d_1)=\J^\sharp(d_2)$ iff $d_1=d_2$.
\end{lemma}
\begin{proof}
It is convenient to give the explicit definition of $\J^\sharp$. Recall that an arrow $d\colon 2^n \to 2^m$ in $\Sets_2^+$ is a subprobability distribution on $\Sets_2[2^n,2^m]$, i.e., an element of $\Dis(\Sets_2[2^n,2^m])$. $\J^\sharp$ is the identity on objects functor mapping $d\colon 2^n \to 2^m$, into the Kleisli arrow defined for all $b\in 2^n, b'\in 2^m$ as $\J^\sharp(d)(b'|b)=\sum_{\{f\mid f(b)=b'\}}d(f)$. It is trivial to see that for $n=0$, $\J^\sharp$ provides the obvious bijection $$\Dis(\Sets_2[1,2^m])\cong \Dis(2^m) \cong   \KlD_2[1,2^m]\text{.}$$
%
%$b=\bullet$ (recall that $\bullet$ is the unique element of $1$), $J^\sharp(d)(b'|\bullet)=\sum_{\{f\mid f(\bullet)=b'\}}d(f)$.
%Define $U\colon \KlD_2[1,2^m] \to \Sets_2^+[1,2^m]$ as the function mapping any $g\colon 1 \to \Dis(2^m)$ into $\sum_{b'\in 2^m} g(b'|\bullet)\cdot \bar{b'}$ where $\bar{b'}\colon 1 \to 2^m$ is the function mapping $\bullet$ into $b'$. It is immediate to see that $U$ and $J^\sharp$ provides the obvious bijection $\Dis(\Sets_2[1,2^m])\cong \KlD_2[1,2^m]$.
\end{proof}
\end{comment}
%
%
Since $\eqsynq{Q}$ is the identity on objects and $G$ is full and faithful, then by the properties of orthogonal factorisation systems (see e.g. \cite{nlab:bofactorizationsystem}), there exists a unique $H\colon  \eqsynq{\CatT{\Diag{\ThB}}} \to \stmat{\KlD_2}$ making the above diagram commute. Below we prove that $H$ is faithful to conclude that also $I$ is faithful.


We first prove that $F$ is faithful on vectors of Booleans.
\begin{lemma}\label{lemma:Ffaith}
For all $\t,\t'\in \CatT{\Diag{\ThB}}[A^0,A^m]$, if $F(\t)=F(\t')$, then $\t=\t'$.
\end{lemma}



Now, by relying on Lemma~\ref{lemma:caratterizzazionecircuiti0n}, we have the following normal forms for tapes $\t \colon A^0 \to A^m$.

\begin{lemma}\label{lemma:PBP0}
For all  $\t\in \CatT{\Diag{\ThPB}}[A^0,A^m]$, there exist, for  $i=1,\dots,n$,  $p_i\in (0,1)$ such that $\sum_{i=1}^{n}p_i= 1$, $\overrightarrow{b}_i\in \Cat{B}[1,A^m]$ and $p,q\in [0,1]$ such that $$\t=(\sum_{i=1}^{n}p_i\cdot \overrightarrow{b}_i)+_p(\star_{A^0,A^m} +_q \Flipm{\bot}[t])\text{.}$$ 
  \end{lemma}


The previous two results, combined with Lemma~\ref{lemma:bottomstar2} allow us to prove the following key property.

\begin{lemma}\label{lemma:PBP1}
  For all $\t,\t'\in \CatT{\Diag{\ThPB}}[A^0,A^m]$, if $F(\t)=F(\t')$, then $\t\sim \t'$.
\end{lemma}





\begin{theorem}\label{thm:completenessPBPtapes}
  $H\colon \eqsynq{\CatT{\Diag{\ThPB}}} \to \stmat{\KlD_2}$ is faithful.%\marginpar{Il Codminio di $H$ e' sbagliato}
\end{theorem}
\begin{proof}
  Let $[\t]_\sim, [\s]_\sim \in \eqsynq{\CatT{\Diag{\ThPB}}}[A^n,A^m]$ be such that $H([\t]_\sim)=H([\s]_\sim)$. Then, consider the following derivation:
  \begin{align}
    H([\t]_\sim)=H([\s]_\sim) &\implies F(\t)=F(\s) \tag{$F=\eqsynq{Q};H$}\\
    &\implies \text{for all } b\in \Cat{B}[1,A^n], F(b);F(\t)=F(b);F(\s) \notag \\
    &\implies \text{for all } b\in \Cat{B}[1,A^n], F(b;\t)=F(b;\s) \tag{Functoriality}\\
    &\implies \text{for all } b\in \Cat{B}[1,A^n], b;\t \eqsyn b;\s \tag{Lemma \ref{lemma:PBP1}}\\
    &\implies \t \eqsyn \s \tag{Lemma \ref{lemma:PBP2}}
  \end{align}
  Hence, $[\t]_\sim=[\s]_\sim$. The above derivation proves that $H$ is faithful for arrows of type $A^n \to A^m$. For arrows of type $ A^k \to \bigoplus_{i=1}^nA^{m_i}$ one can rely on convex products and reduce to the previous case. While for arrows of arbitrary type $\bigoplus_{j=1}^o A^{k_j} \to \bigoplus_{i=1}^nA^{m_i}$, one can easily rely on the universal property of coproducts, see Appendix~\ref{app:{sec:completenessprobbooltapes}}
 for more details.
\end{proof}

\begin{corollary}\label{cor:completenessPBPtapes}
  For all $\s,\t \in \CatT{\Diag{\SigPB}}$, if $\dsem{\s}=\dsem{\t}$ then $\s \eqsynbis \t$.
\end{corollary}




